Modular Linear Differential Equations for Hecke and Fricke Groups

Modular linear differential equations (MLDE) play a significant role in the classification of two-dimensional CFTs, where the modular forms in the equations belonged to the space of $\text{SL}(2,\mathbb{Z})$. A systematic study of the differential equations and their solutions for the Hecke groups $\Gamma_{0}(N)$ and Fricke groups $\Gamma_{0}^{+}(N)$ would better our understanding of CFT classification as there has not been significant work on the MLDE analysis for subgroups of $\text{SL}(2,\mathbb{Z})$. In this paper, we set up and solve MLDEs for Hecke and Fricke groups at levels $N\leq 12$ and report on admissible character-like solutions obtained in each group. We find that only the first four genus zero groups $\Gamma_{0}^{+}(p)$ where $p$ is a prime divisor of the Monster group $\mathbb{M}$ possess admissible single character solutions and we argue that the solutions for $\Gamma_{0}^{+}(11)$ are rendered inadmissible due to its Hauptmodul while those for $\Gamma_{0}^{+}(13)$ are rendered inadmissible due to the nature of the basis decomposition of the space of modular forms. We present a new quasi-character solution at the single character level for the Hecke groups $\Gamma_{0}(2)$, $\Gamma_{0}(7)$, and the subsequent group in its modular tower, $\Gamma_{0}(49)$. We also extend all of the results for single character solutions of Fricke groups to all prime divisor levels of $\mathbb{M}$ and remark on favorable properties in each group that could play a role in obtaining admissible solutions. Finally, we find the $\Theta$-series associated with levels $p = 2,3,5,7$ and the corresponding lattice data of Kissing numbers and lattice radii for each case. We find that the Fricke $\Theta$-series of level $p = 2$ has distinctive ties to the odd Leech lattice in $24$-dimensions.

==> Gamma_0_4+.tex <==
\section{\texorpdfstring{$\Gamma_{0}^{+}(4)$}{Lg} (note: section yet to be completed){Γ0(4)+}}
A non-zero $f\in\mathbb{M}^{!}_{k}(\Gamma_{0}^{+}(4))$ satisfies the following valence formula
\begin{align}
    \nu_{\infty}(f) + \nu_{-\tfrac{1}{2}}(f) + \frac{1}{2}\nu_{\tfrac{i}{2}}(f) + \sum\limits_{\substack{p\in\Gamma_{0}^{+}(4)\backslash\mathbb{H}^{2}\\ p\neq \tfrac{i}{2}}}\nu_{p}(f) =   \frac{k}{4}.
\end{align}
Using the group data in $\ldots$, we obtain the following Riemann-Roch theorem
\begin{align}
    \begin{split}
        \sum\limits_{i=0}^{n-1}\alpha_{i} =& -\frac{nc}{24} + \sum\limits_{i}\Delta_{i}\\
        =&\frac{1}{4}n(n-1) - \frac{1}{2}\ell.
    \end{split}
\end{align}
From this for $n = 1$, we find the following relation  between the number of zeros in the fundamental domain and the central charge
\begin{align}
    c = 12\ell.
\end{align}
The space of modular forms of $\Gamma_{0}^{+}(4)$ has the following basis decomposition
\begin{align}\label{basis_decomposition_Gamma_0_4+}
    \mathcal{M}_{4n}(\Gamma_{0}^{+}(4)) =& \mathbb{C}\left(\Delta_{4,4^{+}}^{\infty}\right)^{n} \oplus \mathbb{C}\left(\Delta_{4,4^{+}}^{\infty}\right)^{n-1}\Delta_{4,4^{+}}^{-\tfrac{1}{2}}\oplus\ldots\oplus\mathbb{C}\left(\Delta_{4,4^{+}}^{-\tfrac{1}{2}}\right)^{n}, n\in\mathbb{Z},
\end{align}
where
\begin{align}
    \begin{split}
        \Delta_{4,4^{+}}^{\infty}(\tau) =& \left(\frac{\eta(4\tau)\eta(\tau)}{\eta(2\tau)}\right)^{8}\in\mathcal{M}_{4}(\Gamma_{0}(4)),\\
        =& q - 8 q^2 + 28 q^3 - 64 q^4+ \ldots,\\
        \Delta_{4,4^{+}}(\tau) =& \left(\frac{\eta^{4}(2\tau)}{\eta(4\tau)\eta(\tau)}\right)^{8}\in\mathcal{S}_{8}(\Gamma_{0}^{+}(4))\\
        =& q + 8 q^2 + 12 q^3 - 64 q^4 + \ldots
    \end{split}
\end{align}


--------------------------------------------
vestigial stuff:

The following are the modular forms and their $q$-series expansion of this group \cite{Schimannek}
\begin{align}
 \begin{split}
     E_{3,1}(\tau) =& \left(\frac{\eta^{9}(\tau)}{\eta^{3}(3\tau)} + 27\frac{\eta^{9}(3\tau)}{\eta^{3}(\tau)}\right)^{\tfrac{1}{3}}\in\mathcal{M}_{1}(\Gamma_{1}(3))\\
     =& 1 + 6q + 6q^{3} + 6q^{4} + \ldots,\\
     E_{3,3}(\tau) =& \frac{\eta^{9}(3\tau)}{\eta^{3}(\tau)}\in\mathcal{M}_{3}(\Gamma_{1}(3))\\
     =& q + 3q^{2} + 9q^{3} + 13q^{4} + \ldots,\\
     \Delta_{6}(\tau) =& E_{3,3}^{2}(\tau)\in\mathcal{S}_{6}(\Gamma_{1}(3))\\
     =& q + 3 q^2 + 9 q^3 + 13 q^4 + \ldots,\\
     \Delta_{6^{'}}(\tau) =& \left(E_{3,1}^{3}(\tau) - 27E_{3,3}(\tau)\right)^{2}\in\mathcal{S}_{6}(\Gamma_{1}(3))\\
     =& 1 - 18 q + 135 q^2 - 504 q^3 + 657 q^4 + \ldots
 \end{split}   
\end{align}


\subsection*{\texorpdfstring{$\ell = 0$}{Lg}}
Let us consider the simple case with no poles $\ell = 0$ and a single character. The spaces $\mathcal{M}_{0}(\Gamma_{1}(5))$ and $\mathcal{M}_{2}(\Gamma_{1}(5))$ are one- and three-dimensional respectively and hence, we make the following choice
\begin{align}
    \begin{split}
        \omega_{0}(\tau) =& E_{5,1,a}(\tau),\\
        \omega_{2}(\tau) =& \mu E_{5,1,a}^{3}(\tau).
    \end{split}
\end{align}
Since $\mu = 0$, the only solution is the trivial one, $f_{0}(\tau) = 1$. 


\subsection*{\texorpdfstring{$\ell = 1$}{Lg}}
An admissible theory would have a central charge $c = 48$. Since the space $\mathcal{M}_{4}(\Gamma_{1}(5))$ is five-dimensional, we choose $\omega_{4}(\tau) = \mu E_{1,5,a}^{5}(\tau)$. This gives us the following choices for the ratio $\tfrac{\omega_{4}(\tau)}{\omega_{2}(\tau)}$,
\begin{align}
    \begin{split}
        \frac{\omega_{4}(\tau)}{\omega_{2}(\tau)} =& \mu E_{5,1,a}^{2}(\tau)\\
        =& \mu\left(1 + 6 q + 17 q^2 + 28 q^3 + 30 q^4 + \ldots\right)
    \end{split}
\end{align}
The solution to the MLDE takes the following form
\begin{align}
    \chi^{(\ell = 1)}(\tau) = 
\end{align}

 For example, considering only the second choice the first few coefficients of the solution read $m_{1}(\mu) = 6$, $m_{2}(\mu) = 9$, $m_{3}(\mu) = -16$, $m_{3}(\mu) = -36$, $m_{4}(\mu) = -\tfrac{126}{5}$, $\ldots$ thus making the solution inadmissible. The same fate is also shared for solutions at $\ell = 2,3,4,5,6$. Hence, we conclude that there exists no single character solutions for $\ell\leq 6$ in $\Gamma_{0}(3)$.

The ring of modular forms is generated by two weight one modular forms \cite{Schimannek}
\begin{align}
    \begin{split}
        E_{5,1,a}(\tau) =& 1 + 3q + 4q^{2} + 2q^{3} + q^{4} + \ldots\\
        E_{5,1,b}(\tau) =& q - 2q^{2} + 4q^{3} - 3q^{4} + \ldots
    \end{split}
\end{align}







Similarly, for $\Gamma_{0}^{+}(7)$, we have
\begin{align}
    \begin{split}
        &\eta^{48}\left(j_{7^{+}}+ 15+ a\right)\left(j_{7^{+}}+ 15+ b\right)(\tau)\\
        = 1 +& (a+b)q + (-1092 - 24 (a + b) + a b)q^{2}\\
        +& (7112 - 21 (a + b) - 48 a b)q^{3} +  \ldots
    \end{split}
\end{align}
This can be rewritten as follows
\begin{align}
    \begin{split}
        &\eta^{48}\left(j_{7^{+}}+ 15+ a\right)\left(j_{7^{+}}+ 15+ b\right)(\tau)\\
        = 1 +& a_{1}q + a_{2}q^{2} + (45304 - 1173a_{1} - 48 a_{2} - a_{3})q^{3} + \ldots
    \end{split}
\end{align}
Setting $a_{1} = a_{2} = a_{3} = 0$, we find kissing number $\mathscr{K} = 45304$ and lattice radius $\rho = \tfrac{\sqrt{3}}{2}$.
---------------------------------------------
two-character $\Gamma^{+}_{0}(2)$ vestigial stuff:
\subsection*{\texorpdfstring{$\ell = 2$}{Lg}}
The MLDE in this case takes the following form
\\
\begin{align}
    \left[\omega_{4}(\tau)\mathcal{D}^{2} + \omega_{6}(\tau)\mathcal{D} + \omega_{8}(\tau)\right]f(\tau) = 0
\end{align}
\\
Using \ref{number_of_parameters_Gamma_0_2+}  we see that we have three free parameters to deal with here. We make the following choices for $\omega_{4}(\tau)$, $\omega_{6}(\tau)$, and $\omega_{8}(\tau)$,
\begin{align}
    \begin{split}
        \omega_{4}(\tau) =& \mu_{1}E_{4}^{(2^{+})}(\tau),\\
        \omega_{6}(\tau) =& \mu_{2}E_{6}^{(2^{+})}(\tau),\\
        \omega_{8}(\tau) =& \mu_{3}\left(E_{4}^{(2^{+})}\right)^{2}(\tau).
    \end{split}
\end{align}
Making these substitutions, the MLDE reads
\begin{align}\label{l=2_MLDE_Gamma_0_2+}
        \left[\Tilde{\partial}^{2} - \frac{1}{6}E_{2}\Tilde{\partial} + \frac{\mu_{2}}{\mu_{1}}\left(\frac{E_{6}^{(2^{+})}}{E_{4}^{(2^{+})}}\right)\Tilde{\partial} + \frac{\mu_{3}}{\mu_{1}}E_{4}^{(2^{+})}\right]f(\tau) = 0.
\end{align}
We make the following series substitutions to the MLDE in addition to that of $f(\tau)$, $E_{k}(\tau)$, and $E_{4}^{(2^{+})}(\tau)$ defined in \ref{series_defs_Gamma_0_2+},
\begin{align}
    \begin{split}
        \left(\frac{E_{6}^{(2^{+})}}{E_{4}^{(2^{+})}}\right)(\tau) =& \sum\limits_{n=0}^{\infty}\mathfrak{a}_{n}q^{n}\\
        =&1 - 104 q + 2072 q^2 - 49568 q^3 + 1146904 q^4 + \ldots
    \end{split}
\end{align}
These substitutions yield
\\
\begin{align}
    q^{\alpha}\sum\limits_{n=0}^{\infty}f_{n}q^{n}\left[(n + \alpha)^{2} + \sum\limits_{m=0}^{\infty}\left((n + \alpha)\left(\frac{\mu_{2}}{\mu_{1}}\mathfrak{a}_{m}-\frac{1}{6}E_{2,m}\right) + \frac{\mu_{3}}{\mu_{1}}E_{4,m}^{(2^{+})}\right)q^{m} \right] = 0.
\end{align}
For $n=0,m=0$, the indicial equation reads
\begin{align}\label{alpha_0,1_l=2}
    \begin{split}
        &\alpha^{2} + \alpha\left(\frac{\mu_{2}}{\mu_{1}} - \frac{1}{6}\right) + \frac{\mu_{3}}{\mu_{1}}  = 0,\\
        &\alpha_{0} = \frac{1}{2}\left(-\Tilde{\mu}_{(21)} - \sqrt{\Tilde{\mu}_{(21)}^{2} - 4\frac{\mu_{3}}{\mu_{1}}}\right),\\
        &\alpha_{1} = \frac{1}{2}\left(-\Tilde{\mu}_{(21)} + \sqrt{\Tilde{\mu}_{(21)}^{2} - 4\frac{\mu_{3}}{\mu_{1}}}\right),
    \end{split}
\end{align}
where $\Tilde{\mu}_{(21)} = \tfrac{\mu_{2}}{\mu_{1}} - \tfrac{1}{6}$.
Employing identity \ref{Riemann_Roch_Gamma_0_2+}, with $n = 2$ and $\ell = 2$ yields
\\
\begin{align}\label{RR_alpha_0,1_l=2}
    \alpha_{0} + \alpha_{1} =-\frac{1}{4}.
\end{align}
From \ref{alpha_0,1_l=2}, we get $\alpha_{0} + \alpha_{1} = -\Tilde{\mu}_{(21)}$ and \ref{RR_alpha_0,1_l=2} implies $\tfrac{\mu_{2}}{\mu_{1}} = \tfrac{5}{12}$. The MLDE now reads
\begin{align}
     \left[\Tilde{\partial}^{2} - \frac{1}{6}E_{2}\Tilde{\partial} + \frac{5}{12}\left(\frac{E_{6}^{(2^{+})}}{E_{4}^{(2^{+})}}\right)\Tilde{\partial} + \frac{\mu_{3}}{\mu_{1}}E_{4}^{(2^{+})}\right]f(\tau) = 0.
\end{align}
We find the following recursion relation
\begin{align}\label{recursion_Gamma_0_2+_l=2}
    f_{n} = \left((n + \alpha)^{2} + \frac{1}{4}(n + \alpha) + \frac{\mu_{3}}{\mu_{1}} \right)^{-1}\sum\limits_{m=1}^{n}\left(\frac{(n + \alpha - m)}{6}\left(E_{2,m} - \frac{5}{2}\mathfrak{a}_{m}\right) - \frac{\mu_{3}}{\mu_{1}}E_{4,m}^{(2^{+})}\right)f_{n-m}.
\end{align}
When $n=1$, we obtain the following ratio
\begin{align}\label{m_i}
    m_{1}^{(i)} \equiv \frac{f_{1}^{(i)}}{f_{0}^{(i)}} = \frac{8\alpha_{i}(72\alpha_{i} + 77)}{3(8\alpha_{i} + 5)}.
\end{align}
For $i=0,1$. When $i=0$, $\alpha_{0} = -\tfrac{c}{24}$ and we get
\begin{align}
    m_{1}^{(0)} = \frac{c(3c-77)}{3(c-15)},
\end{align}
or equivalently, 
\begin{align}
    3c^{2} - c(77 + 3m_{1}) = -45m_{1}.
\end{align}
where we have dropped the script associated with $i = 0$. Since $m_{1}\in\mathbb{Z}$, at least one of the roots is rational and hence, we set
\begin{align}\label{recast_2}
  (3m_{1} +13)^{2} + 5760 = k^{2},
\end{align}
where $k\in\mathbb{Z}$. Defining
\begin{align}
    p \equiv 5760 + 3m_{1} - k,
\end{align}
we can recast \ref{recast_2} as follows
\begin{align}
    3m_{1} + 13 = \frac{p^{2} - 5760}{2p} = -\frac{2880}{p} + \frac{p}{2}.
\end{align}
This tells us that $p$ must be a negative even integer that divides $2880$ with $0<\vert p\vert<72$ so as to ensure $m_{1}\geq 0$. The list of such values reads $p = -\{2,4,6,8,10,12,16,18,20,24,30,32,36$
$,40,48,60,64\}$. We can rule out $p = -\{2,6,8,12,20,24,30,32,36,48,60\}$ since these yield fractional values for $m_{1}$. This leaves us with $p=-\{4,10,16,18,40,64\}$. From \ref{alpha_0,1_l=2}, we can rewrite $\alpha_{0} =-\tfrac{1}{12}(5+x)$ and $\alpha_{1} = -\tfrac{1}{12}(5-x)$ where $x \equiv \sqrt{25 - 576\tfrac{\mu_{4}}{\mu_{1}}} $ so that the central charge and the conformal dimension can be found to be
\begin{align}\label{c_h}
    c = x + 5,\ \Delta = \frac{x}{12}.
\end{align}
The smaller solution $\alpha_{0}$ corresponds to the identity character and substituting this in \ref{m_i} yields
\begin{align}
    \begin{split}
       m_{1} =& \frac{(5+x)(3x-62)}{3(10-x)},\\
        x =& \frac{1}{6}\left(47 - 3m_{1} \pm \sqrt{9m^{2}_{1}+78m_{1}+5929}\right).
    \end{split}
\end{align}
Using the positive root of $x$ in \ref{c_h}, we obtain a list of CFT data for permissible values of $m_{1}$. This is tabulated in table \ref{tab:theory_Fricke_2_l=2}.
\\
\begin{table}[htb!]
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    $p$ & $c$ & $\Delta$ & $\alpha_{0}$ & $\alpha_{1}$ & $m_{1}^{(0)}$\\
    \hline & & & & &  \\
    -4  & $\tfrac{47}{3}$ & $\tfrac{8}{9}$ & $-\tfrac{47}{72}$ & $\tfrac{17}{72}$ & 235\\
    -10 & $\tfrac{50}{3}$ & $\tfrac{35}{36}$ & $-\tfrac{25}{36}$ & $\tfrac{5}{18}$ & 90\\
    -16 & $\tfrac{53}{3}$ & $\tfrac{19}{18}$ & $-\tfrac{53}{72}$ & $\tfrac{23}{72}$ & 53\\
    -18 & 18 & $\tfrac{13}{12}$ & $-\tfrac{3}{4}$ & $\tfrac{1}{3}$ & 46\\
    -40 & $\tfrac{65}{3}$ & $\tfrac{25}{18}$ & $-\tfrac{65}{72}$ & $\tfrac{35}{72}$ & 13\\
    -64 & $\tfrac{77}{3}$ & $\tfrac{31}{18}$ &  $-\tfrac{77}{72}$ & $\tfrac{47}{72}$ & 0\\
    \end{tabular}
    \caption{$c$ and $\Delta$ data corresponding to the Fricke group $\Gamma_{0}^{+}(2)$ with $\ell = 2$.}
    \label{tab:theory_Fricke_2_l=2}
\end{table}
\\
We now compute $m_{2}^{(0)}$ using the recursion relation \ref{recursion_Gamma_0_2+_l=2}. If this turns out to be negative or fractional, then we rule out the theory's candidature. When $n=2$, we have
\begin{align}
    m_{2}^{(i)} \equiv \frac{f_{2}^{(i)}}{f_{0}^{(i)}} = \frac{\alpha_{i}\left(4044\alpha_{i} - 4241\frac{\mu_{4}}{\mu_{1}}\right)}{3(8\alpha_{i} + 9)} - \frac{4m_{1}^{(i)}\left(59 + \alpha_{i}(77 + 72\alpha_{i})\right)}{3(8\alpha_{i} + 9)}.
\end{align}
For $i=0$, we find that the values of $m_{2}^{(0)}$ corresponding to our candidate theories to yield (positive) fractional values for all the listed central charges in \ref{tab:theory_Fricke_2_l=2}. We rule these theories out and conclude that there exists no CFTs at $\ell = 2$. It is also interesting to note that there is no single character theory with $\ell = 2$.


\subsection*{\texorpdfstring{$\ell = 3$}{Lg}}
The MLDE in this case reads
\begin{align}
    \left[\omega_{6}(\tau)\mathcal{D}^{2} + \omega_{8}(\tau)\mathcal{D} + \omega_{10}(\tau)\right]f(\tau) = 0.
\end{align}
Using \ref{number_of_parameters_Gamma_0_2+} we determine the number of free parameters to be three. We make the following choices for modular forms $\omega_{6}(\tau)$, $\omega_{8}(\tau)$, and $\omega_{10}(\tau)$,
\begin{align}
    \begin{split}
        \omega_{6}(\tau) =& \mu_{1}E_{6}^{(2^{+})}(\tau),\\
        \omega_{8}(\tau) =& \mu_{2}\left(E_{4}^{(2^{+})}\right)^{2}(\tau),\\
        \omega_{10}(\tau) =& \mu_{3}E_{10}^{(2^{+})}(\tau).
    \end{split}
\end{align}
Making these substitutions, we have
\begin{align}
    \left[\Tilde{\partial}^{2} + \left(\frac{\mu_{2}}{\mu_{1}}\frac{\left(E^{(2^{+})}_{4}\right)^{2}}{E_{6}^{(2^{+})}} - \frac{1}{6}E_{2}\right)\Tilde{\partial} + \frac{\mu_{3}}{\mu_{1}}\frac{E^{(2^{+})}_{10}}{E_{6}^{(2^{+})}}\right]f(\tau) = 0.
\end{align}
We make the following substitutions to the MLDE in addition to that of $f(\tau)$ and $E_{k}(\tau)$ defined in \ref{series_defs_Gamma_0_2+},
\begin{align}
    \begin{split}
        \left(\frac{\left(E_{4}^{(2^{+})}\right)^{2}}{E_{6}^{(2^{+})}}\right)(\tau) =& \sum\limits_{n=0}^{\infty}\mathfrak{b}_{n}q^{n}\\
        =& 1 + 152 q + 14360 q^2 + 1229408 q^3 + 104497176 q^4 + \ldots,\\
        \left(\frac{E_{10}^{(2^{+})}}{E_{6}^{(2^{+})}}\right)(\tau) =& \sum\limits_{n=0}^{\infty}\mathfrak{c}_{n}q^{n}\\
        =& 1 + 48 q + 624 q^2 + 1344 q^3 + 5232 q^4 + \ldots.
    \end{split}
\end{align}
These substitutions yield
\begin{align}
    q^{\alpha}\sum\limits_{n=0}^{\infty}f_{n}q^{n}\left[(n + \alpha)^{2} + \sum\limits_{m=0}^{\infty}\left((n + \alpha)\left(\frac{\mu_{2}}{\mu_{1}}\mathfrak{b}_{m} - \frac{1}{6}E_{2,m}\right) + \frac{\mu_{3}}{\mu_{1}}\mathfrak{c}_{m}\right)q^{m}\right] = 0.
\end{align}
For $n=0,m=0$, we obtain the same indicial equation and roots as in \ref{alpha_0,1_l=2}. Now, using the Riemann-Roch identity \ref{Riemann_Roch_Gamma_0_2+}, with $n = 2$ and $\ell = 3$, we get
\begin{align}
    \alpha_{0} + \alpha_{1} = -\frac{1}{2}.
\end{align}
From this, we see that $\frac{\mu_{2}}{\mu_{1}} = \tfrac{2}{3}$. We find the following recursion relation, in this case,
\begin{align}
    f_{n} = \left((n + \alpha)^{2} + \frac{1}{2}(n + \alpha) + \frac{\mu_{3}}{\mu_{1}}\right)^{-1}\sum\limits_{m=1}^{n}\left(\frac{(n + \alpha - m}{6}\left(E_{2,m} -4\mathfrak{b}_{m}\right) - \frac{\mu_{3}}{\mu_{1}}\mathfrak{c}_{m}\right)f_{n-m}.
\end{align}
When $n = 1$, the ratio $m_{1}^{(i)}$ reads
\begin{align}\label{m_i_l=3}
    m_{1}^{(i)} \equiv \frac{f_{1}^{(i)}}{f_{0}^{(i)}} = \frac{8\alpha_{i}(36\alpha_{i} - 61)}{12\alpha{i} + 9}.
\end{align}
For $i = 0,1$. When $i = 0$ with $\alpha_{0} = -\tfrac{c}{24}$, we have
\begin{align}
    m_{1}^{(0)} = \frac{c(122 + 3c)}{3(18-c)}.
\end{align}
This tells us that $c$ is bounded by $18$ above in order for $m_{1}\geq 0$. Dropping the script associated with $i = 0$, we can rewrite this equation as follows
\begin{align}
    3c^{2} + c(122 + 3m_{1}) = 54m_{1}.
\end{align}
We now set
\begin{align}\label{recast_3}
    (3m_{1} + 230)^{2} - 38016 = k^{2},\ k\in\mathbb{Z}.
\end{align}
Now, defining
\begin{align}
    p\equiv 230 + 3m_{1} - k,
\end{align}
we can recast \ref{recast_3} as follows
\begin{align}
    3m_{1} + 230 = \frac{19008}{p} + \frac{p}{2}.
\end{align}
This tells us that $p$ must be a positive even integer that divided $19008$ with $0<p<132$ so as to ensure $m_{1}\geq 1$. The list of such values if $p= \left\{4, 16, 22, 64, 88, 108\right\}$. From \ref{alpha_0,1_l=2}, we can rewrite $\alpha_{0} =-\tfrac{1}{4}(1+x)$ and $\alpha_{1} = -\tfrac{1}{4}(1-x)$ where $x \equiv \sqrt{1 - 4\tfrac{\mu_{4}}{\mu_{1}}} $ so that the central charge and the conformal dimension can be found to be
\begin{align}\label{c_h_l=3}
    c = 6(1 + x),\ \Delta = \frac{x}{2}.
\end{align}
Substituting the smaller solution $\alpha_{0}$ in \ref{m_i_l=3} yields
\begin{align}
    \begin{split}
        m_{1} =& \frac{2(1 + x)(9x + 70)}{3(x-2)},\\
        x =& \frac{1}{36}\left(-158 - 3m_{1} \pm \sqrt{9m_{1}^{2} + 1380m_{1} +14884}\right).
    \end{split}
\end{align}
Using the positive root of $x$, we obtain a list of CFT data for permissible values of $m_{1}$ (see table \ref{tab:theory_Fricke_2_l=3}) where we have omitted the data corresponding to $p = 88, 108$ since the conformal dimensions are negative.
\\
\begin{table}[htb!]
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    $p$ & $c$ & $\Delta$ & $\alpha_{0}$ & $\alpha_{1}$ & $m_{1}^{(0)}$\\
    \hline & & & & &  \\
    4  & $\tfrac{52}{3}$ & $\tfrac{17}{18}$ & $-\tfrac{13}{18}$ & $\tfrac{2}{9}$ & 1508\\
    16  & $\tfrac{46}{3}$ & $\tfrac{7}{9}$ & $-\tfrac{23}{36}$ & $\tfrac{5}{36}$ & 322\\
    22  & $\tfrac{43}{3}$ & $\tfrac{25}{36}$ & $-\tfrac{43}{72}$ & $\tfrac{7}{72}$ & 215\\
    64  & $\tfrac{22}{3}$ & $\tfrac{1}{9}$ & $-\tfrac{11}{36}$ & $-\tfrac{7}{36}$ & 33\\
    \end{tabular}
    \caption{$c$ and $\Delta$ data corresponding to the Fricke group $\Gamma_{0}^{+}(2)$ with $\ell = 3$.}
    \label{tab:theory_Fricke_2_l=3}
\end{table}
We rule these candidate theories out since the ratio $m_{2}^{(0)}$ is a negative fraction for the cases corresponding to $p = \left\{4,16,22\right\}$ and a positive fraction for the case corresponding to $p = 64$. Hence, we conclude that there are no two-character CFTs at $\ell = 3$ which again matches with the fact that we did not find any single character theories with $\ell = 3$.



\subsection*{\texorpdfstring{$\ell = 4$}{Lg}}
The MLDE in this case reads
\begin{align}
    \left[\omega_{8}(\tau)\mathcal{D}^{2} + \omega_{10}(\tau)\mathcal{D} + \omega_{12}(\tau)\right]f(\tau) = 0.
\end{align}
Using \ref{number_of_parameters_Gamma_0_2+} we determine the number of free parameters to be three. We make the following choices for modular forms $\omega_{6}(\tau)$, $\omega_{8}(\tau)$, and $\omega_{10}(\tau)$,
\begin{align}
    \begin{split}
        \omega_{8}(\tau) =& \mu_{1}\left(E_{4}^{(2^{+})}\right)^{2}(\tau),\\
        \omega_{10}(\tau) =& \mu_{2}E_{10}^{(2^{+})}(\tau),\\
        \omega_{12}(\tau) =& \mu_{3}\left(E_{4}^{(2^{+})}\right)^{3}(\tau).
    \end{split}
\end{align}
Making these substitutions, we have
\begin{align}
    \left[\Tilde{\partial}^{2} + \left(\frac{\mu_{2}}{\mu_{1}}\frac{E_{10}^{(2^{+})}}{\left(E_{4}^{(2^{+})}\right)^{2}} - \frac{1}{6}E_{2}\right)\Tilde{\partial} + \frac{\mu_{3}}{\mu_{1}}E^{(2^{+})}_{4}\right]f(\tau) = 0.
\end{align}
In addition to the series substitutions of $f(\tau)$, $E_{k}(\tau)$, and $E_{4}^{(2^{+})}(\tau)$ defined in \ref{series_defs_Gamma_0_2+}, we make the following substitution
\begin{align}
    \left(\frac{E_{10}^{(2^{+})}}{\left(E_{4}^{(2^{+})}\right)^{2}}\right)(\tau) =& \sum\limits_{n=1}^{\infty}\mathfrak{d}_{n}q^{n}\\
    =& 1 - 104 q + 2072 q^2 - 49568 q^3 + 1146904 q^4 + \ldots
\end{align}
We now have
\begin{align}
    q^{\alpha}\sum\limits_{n=0}^{\infty}f_{n}q^{n}\left[(n + \alpha)^{2} + \sum\limits_{m=0}^{\infty}\left((n + \alpha)\left(\frac{\mu_{2}}{\mu_{1}}\mathfrak{d}_{m} - \frac{1}{6}E_{2,m}\right) + \frac{\mu_{3}}{\mu_{1}}E^{(2^{+})}_{4,m}\right)q^{m}\right] = 0.
\end{align}
For $n=0,m=0$, we obtain the same indicial equation as in \ref{alpha_0,1_l=2}. Using the Riemann-Roch identity \ref{Riemann_Roch_Gamma_0_2+}, with $n = 2$ and $\ell = 4$ yields
\begin{align}
    \alpha_{0} + \alpha_{1} = -\frac{3}{4}.
\end{align}
From this we get $\tfrac{\mu_{2}}{\mu_{1}} = \tfrac{11}{12}$. We find the following recursion relation, in this case,
\begin{align}
    f_{n} = \left((n + \alpha)^{2} + \frac{3}{4}(n + \alpha) + \frac{\mu_{3}}{\mu_{1}}\right)^{-1}\sum\limits_{m=1}^{n}\left(\frac{(n + \alpha - m}{6}\left(E_{2,m} -\frac{11}{2}\mathfrak{d}_{m}\right) - \frac{\mu_{3}}{\mu_{1}}E^{(2^{+})}_{4,m}\right)f_{n-m}.
\end{align}
When $n = 1$, the ratio $m_{1}^{(i)}$ reads
\begin{align}\label{m_i_l=4}
    m_{1}^{(i)} \equiv \frac{f_{1}^{(i)}}{f_{0}^{(i)}} = \frac{8\alpha_{i}(36\alpha_{i} - 61)}{12\alpha{i} + 9}.
\end{align}
For $i = 0,1$. When $i = 0$ with $\alpha_{0} = -\tfrac{c}{24}$, we have
\begin{align}
    m_{1}^{(0)} = \frac{c(122 + 3c)}{3(18-c)}.
\end{align}
This tells us that $c$ is bounded by $18$ above in order for $m_{1}\geq 0$. Dropping the script associated with $i = 0$, we can rewrite this equation as follows
\begin{align}
    3c^{2} + c(122 + 3m_{1}) = 54m_{1}.
\end{align}
We now set
\begin{align}\label{recast_4}
    (3m_{1} + 230)^{2} - 38016 = k^{2},\ k\in\mathbb{Z}.
\end{align}
Now, defining
\begin{align}
    p\equiv 230 + 3m_{1} - k,
\end{align}
we can recast \ref{recast_4} as follows
\begin{align}
    3m_{1} + 230 = \frac{19008}{p} + \frac{p}{2}.
\end{align}
This tells us that $p$ must be a positive even integer that divided $19008$ with $0<p<132$ so as to ensure $m_{1}\geq 1$. The list of such values if $p= \left\{4, 16, 22, 64, 88, 108\right\}$. From \ref{alpha_0,1_l=2}, we can rewrite $\alpha_{0} =-\tfrac{1}{4}(1+x)$ and $\alpha_{1} = -\tfrac{1}{4}(1-x)$ where $x \equiv \sqrt{1 - 4\tfrac{\mu_{4}}{\mu_{1}}} $ so that the central charge and the conformal dimension can be found to be
\begin{align}\label{c_h_l=4}
    c = 6(1 + x),\ \Delta = \frac{x}{2}.
\end{align}
Substituting the smaller solution $\alpha_{0}$ in \ref{m_i_l=3} yields
\begin{align}
    \begin{split}
        m_{1} =& \frac{2(1 + x)(9x + 70)}{3(x-2)},\\
        x =& \frac{1}{36}\left(-158 - 3m_{1} \pm \sqrt{9m_{1}^{2} + 1380m_{1} +14884}\right).
    \end{split}
\end{align}
Using the positive root of $x$, we obtain a list of CFT data for permissible values of $m_{1}$ (see table \ref{tab:theory_Fricke_2_l=3}) where we have omitted the data corresponding to $p = 88, 108$ since the conformal dimensions are negative.
\\



==> Gamma_0_4.tex <==
\subsection{\texorpdfstring{$\Gamma_{0}(4)$}{Lg}}
A non-zero $f\in\mathcal{M}^{!}_{k}(\Gamma_{0}^{+}(4))$ satisfies the following valence formula
\begin{align}
    \nu_{\infty}(f) + \nu_{0}(f) + \nu_{-\tfrac{1}{2}}(f) + \sum\limits_{p\in\Gamma_{0}(4)\backslash\mathbb{H}^{2}}\nu_{p}(f) =   \frac{k}{2}.
\end{align}
The dimension of the space of modular forms of $\Gamma_{0}(4)$ is given by (cite Modular Forms
Spring 2011 Notes (and beyond) Kimball Martin p. 90)
\begin{align}
    \begin{split}
        \text{dim}\ \mathcal{M}_{k}\Gamma_{0}(4)) = \begin{cases}
        0,\ &\text{if}\ k<0\ \text{or $k$ is odd},\\
        1 + \frac{k}{2},\ &\text{otherwise}.
        \end{cases}
    \end{split}
\end{align}
Using the group data in $\ldots$, we obtain the following Riemann-Roch theorem
\begin{align}
    \begin{split}
        \sum\limits_{i=0}^{n-1}\alpha_{i} =& -\frac{nc}{24} + \sum\limits_{i}\Delta_{i}\\
        =&\frac{1}{2}n(n-1) - \ell.
    \end{split}
\end{align}
From this for $n = 1$, we find the following relation  between the number of zeros in the fundamental domain and the central charge
\begin{align}
    c = 24\ell.
\end{align}
The space of modular forms of $\Gamma_{0}(4)$ has the following basis decomposition
\begin{align}\label{basis_decomposition_Gamma_0_4}
    \mathcal{M}_{2n}(\Gamma_{0}(4)) =& \mathbb{C}\left(\Delta_{4}^{\infty}\right)^{n} \oplus \mathbb{C}\left(\Delta_{4}^{\infty}\right)^{n-1}\Delta_{4}^{0}\oplus\ldots\oplus\mathbb{C}\left(\Delta_{4}^{0}\right)^{n}, n\in\mathbb{Z},
\end{align}
where
\begin{align}
    \begin{split}
        \Delta_{4}^{\infty}(\tau) =& \left(\frac{\eta^{2}(4\tau)}{\eta(2\tau)}\right)^{4}\in\mathcal{M}_{2}(\Gamma_{0}(4)),\\
        =& q + 4 q^3 + 6 q^5 + \ldots,\\
        \Delta_{4}^{0}(\tau) =& \left(\frac{\eta^{2}(\tau)}{\eta(2\tau)}\right)^{4}\in\mathcal{M}_{2}(\Gamma_{0}(4))\\
        =& 1 - 8 q + 24 q^2 - 32 q^3 + 24 q^4 + \ldots
    \end{split}
\end{align}
The Hauptmodul of $\Gamma_{0}(4)$ is defined as follows
\begin{align}
    \begin{split}
    j_{4}(\tau) =& \left(\frac{\Delta_{4}^{0}}{\Delta_{4}^{\infty}}\right)(\tau) = \left(\frac{\eta(\tau)}{\eta(4\tau)}\right)^{8}\\
    =& q^{-1} - 8 + 20q - 62q^{3} + 216q^{5} + \ldots
    \end{split}
\end{align}
We note here that $j_{4}(\tau)$ is related to the Haputmodul of $\Gamma(2)$ thanks to the isomorphism between the curves $X(2)$ and $X_{0}(4)$. The Hauptmodul of $\Gamma(2)$ is the modular lambda function $\lambda(\tau)$ which possesses the following $q$-series expansion
\begin{align}
    \begin{split}
    \lambda(\tau) =& \left(\frac{\theta_{2}}{\theta_{3}}\right)^{4}(\tau)\\
    =& 16 q - 128 q^2 + 704 q^3 - 3072 q^4 + \ldots
    \end{split}
\end{align}
The relation between $j_{4}(\tau)$ and $\lambda(\tau)$ is a follows
\begin{align}\label{lambda_j_4_relation}
    \lambda(\tau) = \left(1 + \frac{1}{16}j_{4}(\tau)\right)^{-1}.
\end{align}
With $K = \tfrac{12^{3}}{j(\tau)}$ with $j(\tau)$ being the $\text{SL}(2,\mathbb{Z})$ Hauptmodul, the relation between $\lambda(\tau)$ and $j(\tau)$ reads
\begin{align}
    \lambda(\tau)\left(1-\lambda(\tau)\right) = \frac{16}{K + 24}.
\end{align}
From this and \ref{lambda_j_4_relation} we get
\begin{align}\label{j_j_4_relation}
    j(\tau) = \left(\frac{(12)^{3}j_{4}}{j_{4}^{2} + 8j_{4} + 256}\right)(\tau).
\end{align}
Changing variables from $\tau$ to $j(\tau)$, we perform modular re-parameterization so that we can express the Ramanujan-Serre covariant derivatives as follows
\begin{align}
    \begin{split}
        \mathcal{D} =& \theta_{q} = -\left(\frac{E_{6}}{E_{4}}\right)\theta_{j},\\
        \mathcal{D}^{2} =& q^{2}\frac{d^{2}}{dq^{2}} = \left(\frac{E_{6}}{E_{4}}\right)^{2}\left(\theta_{j}^{2} - \frac{2(12)^{3} + j}{6(12^{3} - j)}\theta_{j}\right),
    \end{split}
\end{align}
where we have defined the operator $\theta_{a} \equiv a\tfrac{d}{da}$. Using relation \ref{j_j_4_relation}, we obtain
\begin{align}
    \begin{split}
        \mathcal{D} =& q\frac{d}{dq} = A(j_{4})\theta_{j_{4}},\\
        \mathcal{D}^{2} =& q^{2}\frac{d^{2}}{dq^{2}} = A(j_{4})^{2}\theta_{j_{4}}^{2}  + B(j_{4})\theta_{j_{4}},
    \end{split}
\end{align}
where 
\begin{align}
    A(j_{4}) = -\left(\frac{E_{6}}{E_{4}}\right)\left(\frac{(12)^{6}(j_{4}^{2} - 256)}{(j_{4}^{2} + 8j_{4} + 256)}\right),\ B(j_{4}) = -\left(\frac{E_{6}}{E_{4}}\right)^{2}\frac{(12)^{3}j_{4}(512 + j_{4}(17 + 2j_{4}))}{6(256 + j_{4}(7 + j_{4}))(256 + j_{4}(8 + j_{4}))}.
\end{align}
Now, the $(n,\ell) = (2,0)$ MLDE for $\Gamma_{0}(4)$ takes the following form
\begin{align}
    \left[\mathcal{D}^{2} + \omega_{2}(\tau)\mathcal{D} + \omega_{4}(\tau)\right]f(\tau) = 0,
\end{align}
where the most general choice for the modular forms $\omega_{i}(\tau)$ are the following
\begin{align}
    \begin{split}
        \omega_{2}(\tau) =& \mu_{1}\Delta_{4}^{\infty} + \mu_{2}\Delta_{4}^{0},\\
        \omega_{4}(\tau) =& \mu_{3}\left(\Delta_{4}^{\infty}\right)^{2} + \mu_{4}\left(\Delta_{4}^{\infty}\Delta_{4}^{0}\right) + \mu_{5}\left(\Delta_{4}^{0}\right)^{2}.
    \end{split}
\end{align}
Let us choose $\mu_{1} = \mu_{3} = \mu_{4} = 0$, relabel the free parameters, and substitute for the covariant derivatives to obtain
\begin{align}
    \left[A(j_{4})^{2}\theta_{j_{4}}^{2} + \left(\mu_{1}\Delta_{4}^{0}A(j_{4}) + B(j_{4})\right)\theta_{j_{4}} + \mu_{2}\left(\Delta_{4}^{0}\right)^{2}\right]f(\tau) = 0.
\end{align}

\newpage
We can now use this relation to find the $q$-derivatives of $j_{4}(\tau)$. The $q$-derivative of $\lambda(\tau)$ reads
\begin{align}
    \begin{split}
    q\frac{d}{dq}\lambda(\tau) =& \frac{1}{2\pi i}\frac{d}{d\tau}\lambda(\tau)\\
    =& \frac{1}{2}\theta_{4}^{4}(\tau)\lambda(\tau) = \frac{1}{2}\left(\theta_{3}^{4}(1 - \lambda)\lambda\right)(\tau),\\
    q^{2}\frac{d^{2}}{dq^{2}}\lambda(\tau) =& \frac{1}{(2\pi i)^{2}}\frac{d^{2}}{d\tau^{2}}\lambda(\tau)\\
    =& \left(\frac{1}{2}\theta_{3}^{4}(1-\lambda)\left(\frac{1}{2}\theta_{3}^{4}(1 - \lambda) - 4\right)\lambda\right)(\tau).
    \end{split}
\end{align}
From \ref{lambda_j_4_relation}, we find
\begin{align}
    \begin{split}
        q\frac{d}{dq}j_{4}(\tau) =& \frac{1}{2\pi i}\frac{d}{d\tau}j_{4}(\tau) = -\left(\frac{1}{2}\theta_{4}^{4}\left(16 + j_{4}\right)\right)(\tau),\\
        q^{2}\frac{d^{2}}{dq^{2}}j_{4}(\tau) =& \frac{1}{(2\pi i)^{2}}\frac{d^{2}}{d\tau^{2}}j_{4}(\tau) = \left(\frac{1}{4}\theta_{4}^{4}(16 + j_{4})\left[2\theta_{4}^{4} - \frac{j_{4}(-128 + j_{4}(\theta_{4}^{4} - 8))(16 + j_{4})}{(16 + j_{4})^{3}}\right]\right)(\tau).
    \end{split}
\end{align}
From cite{}, the $(n,\ell) = (3,0)$ MLDE for $\text{SL}(2,\mathbb{Z})$ reads
\begin{align}
    \left[\mathcal{D}^{3} + \mu_{1}E_{4}(\tau)\mathcal{D} + \mu_{2}E_{6}(\tau)\right]f(\tau) = 0.
\end{align}
This can be recast by introducing the parameter $K$ as follows
\begin{align}
    &\left[(1 - K)\left(K^{3}\frac{d^{3}}{dK^{3}}\right) - \left(K + \frac{1}{2}\right)\left(K^{2}\frac{d^{2}}{dK^{2}}\right) + \left(\mu_{1} + \frac{1-4K}{18}\right)\left(K\frac{d}{dK}\right) + \mu_{2}\right]f(\tau) = 0,\\
    &\mu_{1} = \frac{1}{576}\left(3c^{2} - 48c\Delta_{1} - 48c\Delta_{2} + 576\Delta_{1}\Delta_{2} - 32\right),\\
    &\mu_{2} = \frac{c^{3}}{13824} - \frac{c^{2}\Delta_{1}}{576} - \frac{c^{2}\Delta_{2}}{576} + \frac{c\Delta_{1}\Delta_{2}}{24}.
\end{align}
From \ref{lambda_j_4_relation} we find
\begin{align}
    K = \left(\frac{j_{4}^{2} + 8j_{4} + 256}{j_{4}}\right)(\tau).
\end{align}






























==> Klein_quartic.tex <==
\section{The Klein quartic}
In the complex projective space $\mathbb{P}^{2}(\mathbb{C})$, the Klein quartic, denoted by $\mathfrak{X}$ is a curve of genus $3$ described by the following homogeneous equation
\begin{equation}\label{plane_quartic}
    \Phi_{4}(x,y,z) \equiv x^{3}y+y^{3}z+z^{3}x = 0,
\end{equation}
where $\Phi_{4}(x,y,z)$ is called the plane quartic. We can think of the curve as being made up of $24$ heptagons with every $3$ heptagons meeting at a single point. These heptagons form a tiling of the hyperbolic plane and all the $24$ heptagons are equivalent thus giving rise to a $24$-fold symmetry. Additionally, there is a $7$-fold symmetry that comes from rotating the heptagons. In total, we have $24\times 7 = 168$ symmetries. In other words, there are $168$ automorphisms of $\mathfrak{X}$. There also exists another tiling, one with $336$ triangles. The fundamental domain in this case is a $14$-gon tiled by $(2,3,7)$-triangles, where the numbers $2$, $3$, and $7$ represent the angles $\tfrac{\pi}{2}$, $\tfrac{\pi}{3}$, and $\tfrac{\pi}{7}$ of each triangle (see figure \ref{fig: Klein_quartic}).
\begin{figure}[htb!]
    \centering
    \includegraphics[width = 12cm]{Klein_quartic.png}
    \caption{(Left) The hyperbolic plane tiled with regular heptagons each made up of seven triangles. Numbering the heptagons from $1-24$, we can curl this up to obtain a $3$-holed torus with three heptagons meeting at one corner (Right). The figure on the right was first created by Joe Christy using a program called Geomview.}
    \label{fig: Klein_quartic}
\end{figure}
Restricting ourselves to only orientation-preserving symmetries, we are left with half the amount of triangles, i.e. $168$ of them which coincides which is the correct number of automorhisms. The group of symmetries or simply, the automorphism group of $\mathfrak{X}$ is isomorphic to the simple group $G = \text{PSL}(2,\mathbb{F}_{7})$ and is order $168$. Formally, we define
\begin{equation}
    \text{PSL}(2,\mathbb{F}_{7}) = \left\{\left.\begin{pmatrix}a & b c & d\end{pmatrix}\right\vert a,b,c,d\in\mathbb{Z}/7\mathbb{Z}, ad-bc = 1\right\}/\{\pm 1\}.
\end{equation}
Here, $\mathbb{F}_{7} = \{0,1,\ldots, 6\}$ with addition and multiplication rules. The principal congruence subgroup of level $7$ is the normal subgroup $\Gamma(7)$ of $\Gamma(1) = \text{PSL}(2,\mathbb{Z})$ and is defined by the following short exact sequence

\begin{equation}
    1\longrightarrow \Gamma(7)\longrightarrow \Gamma(1)\overset{f}{\longrightarrow}\equalto{\text{PSL}(2,\mathbb{F}_{7})}{\Gamma(1)/\Gamma(7)}\longrightarrow 1,
\end{equation}
where $f(A) = A(\text{mod}\ 7)$. the quotient $Y(7) =  \Gamma(7)\backslash\mathbb{H}^{2}$ is a Riemann surface, since the principal congruence subgroup $\Gamma(7)$ is torsion free, and the modular curve of level $7$ is the compact Riemann surface $X(7) = \Gamma(7)\backslash\mathbb{H}^{2*}$, where $\mathbb{H}^{2*} = \mathbb{H}^{2}\cup \mathbb{P}^{1}(\mathbb{C})$ is the extended upper-half plane. The number of cusps of $\Gamma(N)$ is given by 
\begin{equation}
    \frac{N^{2}}{2}\prod\limits_{p\vert N}\left(1 - \frac{1}{p^{2}}\right).
\end{equation}
where the product is taken over all positive divisors $p$ of $N$. Using this we see that $\Gamma(7)$ has $24$ cusps and these correspond to the $24$ points of valency $7$ on the Klein surface. The modular curve $X(7)$ is isomorphic to $\mathfrak{X}$ and has a genus, $g=3$. Also, we note that $G$ is isomorphic to $\text{PSL}(2,\mathbb{Z}/7\mathbb{Z})$ and there exists an exceptional isomorphism with the group $\text{PGL}(3,\mathbb{F}_{2})$, 
\begin{equation}
    \text{PGL}(3,\mathbb{F}_{3})\cong\equalto{\text{PSL}(2,\mathbb{F}_{7})}{ \Gamma(1)/\Gamma(7)}\cong \text{PSL}(2,\mathbb{Z}/7\mathbb{Z})    
\end{equation}
The group $\text{PSL}(2,\mathbb{Z}/7\mathbb{Z})\cong\Gamma(7)$ is a non-Abelian finite subgroup of $\text{SU}(3)$ of order $168$. The group $\Gamma(7)$ is generated by $S$ and $T$ satisfying the following multiplication rules
\begin{align}
    S^{2} = \left(ST\right)^{3} = T^{7} = \left(ST^{3}\right)^{4} = 1.
\end{align}
The Riemann surface associated with the plane quartic $\Phi_{4}(x,y,z)$ defined by \ref{plane_quartic} with its $24$ points of inflection removed, is uniformized by the variable $\tau\in\mathbb{H}^{2}$ via the formulae
\begin{align}
    \begin{split}
        \frac{\mathfrak{f}_{3}}{\mathfrak{f}_{2}} =& q^{-\frac{1}{7}}\frac{\sum\limits_{m=-\infty}^{\infty}(-1)^{m}\left(q^{\frac{21m^{2}+37m+16}{2}} - q^{\frac{21m^{2}+19m+4}{2}}\right)}{\sum\limits_{n=-\infty}^{\infty}(-1)^{n+1}q^{\frac{21n^{2}+7n}{2}}}\\
        =& q^{-\frac{1}{7}}\left(1 + q^2 - q^3 +q^7 - q^8 + q^9 - q^{10} + \ldots\right),\\
        \frac{\mathfrak{f}_{1}}{\mathfrak{f}_{3}} =& q^{-\frac{4}{7}}\frac{\sum\limits_{m=-\infty}^{\infty}(-1)^{m}\left(q^{\frac{21m^{2}+25m+8}{2}} - q^{\frac{21m^{2}+31m+12}{2}}\right)}{\sum\limits_{n=-\infty}^{\infty}(-1)^{n+1}q^{\frac{21n^{2}+7n}{2}}}\\
        =& -q^{-\frac{4}{7}}\left(q - q^2 + q^4 - q^6 + q^8 - q^9 + q^{11} + \ldots\right),\\
        \frac{\mathfrak{f}_{2}}{\mathfrak{f}_{1}} =& q^{-\frac{2}{7}}\frac{\sum\limits_{m=-\infty}^{\infty}(-1)^{m}\left(q^{\frac{21m^{2}+m}{2}} - q^{\frac{21m^{2}+13m+2}{2}}\right)}{\sum\limits_{n=-\infty}^{\infty}(-1)^{n+1}q^{\frac{21n^{2}+7n}{2}}}\\
        =& q^{-\frac{2}{7}}\left(1 - q + q^5 + q^7 - q^8 - q^{10} + \ldots\right),
    \end{split}
\end{align}
where $q = e^{2\pi i\tau}$ and the forms $\mathfrak{f}_{i}$ possess the following Fourier series expansions \cite{Franc-Mason}
\begin{align}\label{the_three_forms}
    \begin{split}
        \mathfrak{f}_{1} =& \eta^{4}(\tau)\left(\frac{\Delta(\tau)}{E_{4}^{3}(\tau)}\right)^{\frac{17}{42}}\pFq{3}{2}{\frac{17}{42},\frac{31}{42},\frac{15}{14}}{\frac{10}{7},\frac{9}{7}}{\frac{1728\Delta(\tau)}{E_{4}^{3}(\tau)}}\\
        =& -q^{\frac{4}{7}}\left(1 - 4 q + 3 q^2 + 5 q^3 - 5 q^4 - 8 q^6 + 10 q^7 - 4 q^9 + 6 q^{10} + \ldots\right),\\
        \mathfrak{f}_{2} =& \eta^{4}(\tau)\left(\frac{\Delta(\tau)}{E_{4}^{3}(\tau)}\right)^{\frac{5}{42}}\pFq{3}{2}{\frac{5}{42},\frac{19}{42},\frac{11}{14}}{\frac{8}{7},\frac{5}{7}}{\frac{1728\Delta(\tau)}{E_{4}^{3}(\tau)}}\\
        =& q^{\frac{2}{7}}\left(1 - 3 q - q^2 + 8 q^3 - 6 q^5 - 4 q^6 + 2 q^8 + 9 q^{10}+\ldots\right),\\
        \mathfrak{f}_{3} =& \eta^{4}(\tau)\left(\frac{\Delta(\tau)}{E_{4}^{3}(\tau)}\right)^{-\frac{1}{42}}\pFq{3}{2}{-\frac{1}{42},\frac{13}{42},\frac{9}{14}}{\frac{6}{7},\frac{4}{7}}{\frac{1728\Delta(\tau)}{E_{4}^{3}(\tau)}}\\
        =&q^{\frac{1}{7}}\left(1 - 3 q + 4 q^3 + 2 q^4 + 3 q^5 - 12 q^6 - 5 q^7 + 7 q^9 + 16 q^{10} + \ldots\right).
    \end{split}
\end{align}
We note that the ratio $\tfrac{E_{4}^{3}}{\Delta}$ is a modular function since both the forms are of equal weights. Since the Dedekind eta function is a modular form of weight $\tfrac{1}{2}$, the modular forms $\mathfrak{f}_{i}$ are of weight $2$. More succinctly, we can express the forms $\mathfrak{f}_{i}$ as the following product sum
\begin{align}
        \begin{split}
        \mathfrak{f}_{i} =& \mathfrak{e} q^{\frac{a}{7}}\prod\limits_{n=1}^{\infty}\left(1-q^{n}\right)^{3}\left(1-q^{7n}\right)\prod\limits_{\substack{n>0\\ n\equiv \pm n_{0}(\text{mod}\ 7)}}\left(1 - q^{n}\right),\\ \left(\mathfrak{e},a,n_{0}\right) =& \begin{cases}
        (-1,4,1),\ i=1
        (1,2,2),\ i=2
        (1,1,4),\ i=3
        \end{cases}.
        \end{split}
\end{align}
For example, with $i=1$, we obtain 
\begin{align}
    \begin{split}
        \mathfrak{f}_{1} &= -q^{\frac{4}{7}}\prod\limits_{n=1}^{\infty}\left(1-q^{n}\right)^{3}\left(1-q^{7n}\right)\prod\limits_{\substack{n=1\\ n\equiv 1(\text{mod}\ 7)}}^{\infty}\left(1-q^{n}\right)\prod\limits_{\substack{n=1\\ n\equiv -1(\text{mod}\ 7)}}^{\infty}\left(1-q^{n}\right)\\
        &=-q^{\frac{4}{7}}\prod\limits_{n=1}^{\infty}\left(1-q^{n}\right)^{3}\left(1-q^{7n}\right)\cdot(1-q)(1-q^{6})(1-q^{8})(1-q^{13})(1-q^{15})(1-q^{20})(1-q^{22})\ldots\\
        &= -q^{\frac{4}{7}}\left(1 - 4 q + 3 q^2 + 5 q^3 - 5 q^4 - 8 q^6 + 10 q^7 - 4 q^9 + 6 q^{10} + \ldots\right), 
    \end{split}
\end{align}
which precisely matches with the $q$-expansion in \ref{the_three_forms}.


==> Three_character_Gamma_0_2+.tex <==
\subsection{Three-character theories (note: section yet to be completed)}
Let us now consider three character theories with $\ell = 0$. The modular invariant differential equation reads
\begin{align}
    \left[\omega_{0}(\tau)\mathcal{D}^{3} + \omega_{2}(\tau)\mathcal{D}^{2} + \omega_{4}(\tau)\mathcal{D} + \omega_{6}(\tau)\right]f(\tau) = 0.
\end{align}
Since there are no modular forms of weight $2$ in $\Gamma_{0}^{+}(2)$, with choices $\omega_{4}(\tau) =\mu_{1} E_{4}^{(2^{+})}(\tau)$ and $\omega_{6}(\tau) = \mu_{2} E_{6}^{(2^{+})}(\tau)$ and in terms of derivatives $\Tilde{\partial}$, the MLDE reads
\begin{align}
        \left[\Tilde{\partial}^{3} - \frac{1}{6}\left(\Tilde{\partial}E_{2}(\tau)\right)\Tilde{\partial}  - \frac{1}{2}E_{2}\Tilde{\partial}^{2} + \frac{1}{18}E^{2}_{2}\Tilde{\partial} + \mu_{1}E_{4}^{(2^{+})}(\tau)\Tilde{\partial} + \mu_{2}E_{6}^{(2^{+})}(\tau)\right]f(\tau) = 0.
\end{align}
We now make use of the Ramanujan identity for the Eisenstein series, $\Tilde{\partial}E_{2} = \tfrac{E_{2}^{2} - E_{4}}{12}$, to rewrite the MLDE as follows
\begin{align}
    \left[\Tilde{\partial}^{3} + \frac{1}{2}\left(\Tilde{\partial}E_{2}(\tau)\right)\Tilde{\partial}  - \frac{1}{2}E_{2}(\tau)\Tilde{\partial}^{2} + \frac{1}{18}E_{4}(\tau)\Tilde{\partial} + \mu_{1}E_{4}^{(2^{+})}(\tau)\Tilde{\partial} + \mu_{2}E_{6}^{(2^{+})}(\tau)\right]f(\tau) = 0.
\end{align}
We make the following substitution in addition to $f(\tau)$ and $E_{k}(\tau)$, and $E_{4}^{(2^{+})}(\tau)$ defined in \ref{series_defs_Gamma_0_2+},
\begin{align}
    \begin{split}
        E^{(2^{+})}_{6}(\tau) =& \sum\limits_{n=0}^{\infty}E^{(2^{+})}_{6,n}q^{n}\\
        =& 1 - 56 q - 2296 q^2 - 13664 q^3 - 73976 q^4 + \ldots,\\
        \Tilde{\partial}E_{2}(\tau) =& q\frac{d}{dq}E_{2}(\tau) = \sum\limits_{n = 0}^{\infty}\mathfrak{e}_{n}q^{n}\\
        =& 24 q - 144 q^2 - 288 q^3 - 672 q^4 - 720 q^5 + \ldots
    \end{split}
\end{align}
\\
We now have the recursion relation
\begin{align}\label{m_1_equation}
    \begin{split}
    &\left((n + \alpha)^{3} - \frac{1}{2}(n + \alpha)^{2} + \left(\mu_{1} + \frac{1}{18}\right)(n + \alpha) + \mu_{2}\right)f_{n} =\\ &\sum\limits_{m=1}^{n}\left(\frac{(n + \alpha - m)^{2}}{2}E_{2,m}
    - \left(\frac{1}{2}\mathfrak{e}_{m} + \frac{1}{18}E_{4,m} + \mu_{1}E^{(2^{+})}_{4,m}\right) (n + \alpha - m) - \mu_{2}E^{(2^{+})}_{6,m}\right)f_{n-m}.
    \end{split}
\end{align}
For $n = 0$, we get the equation
\begin{align}\label{indicial_cubic}
    \alpha^{3} - \frac{1}{2}\alpha^{2} + \Tilde{\mu}_{1}\alpha + \mu_{2} = 0,
\end{align}
where we have defined $\Tilde{\mu}_{1}\equiv \mu_{1} + \tfrac{1}{18}$. For $n = 1$, we obtain the following ratio
\begin{align}\label{m_1_finding_equation}
    \left(3\alpha^{2} - \frac{287}{18}\alpha + \frac{5}{9} + \mu_{1}\right)m_{1} + \left(12\alpha^{2} + 48\alpha\mu_{1} - \frac{176}{3}\alpha + 56\mu_{2}\right) = 0,
\end{align}
where $ m_{1} \equiv \tfrac{f_{1}}{f_{0}}$. From these equations, we find
\begin{align}
    \begin{split}
        \mu_{1} =& \alpha_{0}\alpha_{1} + \alpha_{1}\alpha_{2} + \alpha_{0}\alpha_{2},\\
        \mu_{2} =& -\alpha_{0}\alpha_{1}\alpha_{2},
    \end{split}
\end{align}
where $\alpha_{i}$ with $i=0,1,2$ are the roots of the cubic equation. With $\mu_{2}$ obtained through the indicial cubic equation, we find the following explicit expression for $\mu_{1}$ from \ref{m_1_equation}
\begin{align}
    \mu_{1} = -\frac{504 \alpha_{0}^{3} + \alpha_{0}^{2}(27m_{1} - 144) + \alpha_{0}(40 + 18m_{1}) + 5m_{1}}{9(m_{1} + 104\alpha_{0})}.
\end{align}
We now consider the outcome of the recursion relation for $n =2$ and substitute the known expressions of $\mu_{1}$ and $\mu_{2}$ to obtain
\begin{align}
    \begin{split}
        0 &=226792\alpha_{0}^{4} + \alpha_{0}^{3}\left(-206784 - 27456m_{1} - 768m_{1}^{2} + 1536m_{2}\right)\\
        &+ \alpha_{0}^{2}\left(15840 - 11064m_{1} - 1104m_{1}^{2} + 3216m_{2}\right)\\
        &+ \alpha_{0}(-820m_{1} - 376m_{1}^{2} + 1880m_{2}+ 18m_{1}m_{2}) - (40m_{1}^{2} - 15m_{1}m_{2}).
    \end{split}
\end{align}
We observe that if we define the variable 
\begin{align}\label{N_def}
    N = -28224\alpha_{0},
\end{align}
then the polynomial equation simplifies to 
\begin{align}\label{poly_quartic}
    \begin{split}
        0 &= N^{4} + \left(25848 + 3432m_{1} + 96m_{1}^{2} - 192m_{2}\right)N^{3}\\ &+\left(55883520 - 39033792m_{1} - 3894912m_{1}^{2}+11346048m_{2}\right)N^{2}\\
        &+ \left(81650903040m_{1} + 37439926272m_{1}^{2} -187199631360m_{2}-1792336896m_{1}m_{2}\right)N\\ 
        &- \left(112415370117120m_{1}^{2} - 42155763793920m_{1}m_{2}\right).
    \end{split}
\end{align}
The integer-root theorem requires $N$ to be an integer. Hence, $N$ is further restricted- it not only has to be rational but also is to be an integer. Since $\alpha_{0} = -\tfrac{c}{24}$, we obtain the relation $c = \tfrac{N}{1176}$ from which we see that the central charge has to be a rational number whose denominator is always $1176$. Substituting $\mu_{1}$ and $\mu_{2}$ in \ref{indicial_cubic}, with the definition of $N$ in \ref{N_def} we get
\begin{align}
    \begin{split}
    0 &=\left(\alpha+\frac{N}{28224}\right)\left((1725954048 N - 468397375488m_{1})\alpha^{2} \right.\\
    &\left.+ (-862977024 N - 61152 N^2 + 234198687744m_{1} + 16595712 N m_{1})\alpha\right.\\
    &\left.+(1176 N^{2}m_{1} - 41489280 Nm_{1} + 234198687744 + N^{3} + 21168N^{2} + 22127616 N)\right).
    \end{split}
\end{align}
We see from this that $\alpha = \alpha_{0} = -\tfrac{N}{28224}$ is one of the solutions. Let us denote the other solutions by $\alpha_{1}$ and $\alpha_{2}$ so that $\alpha_{1} - \alpha_{0}$, and $\alpha_{2} - \alpha_{0}$ are the conformal weights $\Delta_{1}$ and $\Delta_{2}$. Hence, $\alpha_{1}$ and $\alpha_{2}$ should also be rational which implies that the discriminant, which is an integer, has to be the perfect square to be able to result in rational roots. This yields
\begin{align}\label{k_equation}
    \begin{split}
        k^{2} = &22308830199742464m_{1}^{2} - 89463898718208m_{1} N - 3161682284544 m_{1}^{2}N + 26752287744 N^{2}\\
        &+ 12148061184 m_{1}N^{2} + 
        112021056m_{1}^{2}N^{2} - 1834560N^{3} - 373968m_{1}N^{3} - 143N^{4},
    \end{split}
\end{align}
where $k$ is a positive integer. This equation where all the unknown variables $N$, $m_{1}$, and $k$ are positive is known as a Diophantine equation. The roots are found to be
\begin{align}
    \frac{-49787136m_{1} + 183456 N -3528 m_{1}N + +13N^{2} \pm k}{56448(13 N - 3528 m_{1})},
\end{align}
where the smaller solution corresponds to $\alpha_{1}$ and the larger one corresponds to $\alpha_{2}$. We now solve \ref{poly_quartic} for a fixed value of $N$ (chosen among the divisors of $28224$) and obtain the solution set $(N,m_{1},m_{2})$. Now, we choose those values of $m_{1}$ and $N$ that result in positive integer values for $k$ that satisfies \ref{k_equation}. By following this procedure, we would have found values for $N$, $m_{1}$, $m_{2}$, and $k$, all of which simultaneously solve equations \ref{poly_quartic} and \ref{k_equation}. The only solution we could find was at $N = 14112$ for which we obtain the values listed in table \ref{tab:N_value}
\\
\begin{table}[htb!]
    \centering
    \begin{tabular}{c|c|c|c}
    $N$ & $m_{1}$ & $m_{2}$ & $k$\\
    \hline & & & \\
    %7056 & 34 & 5 & \\
    14112 & 58 & 66 & 796594176\\
    \end{tabular}
    \caption{Simultaneous solution for $0< N\leq 28224$.}
    \label{tab:N_value}
\end{table}
\\
For the above values, we find roots
\begin{align}
    (\alpha_{0},\alpha_{1},\alpha_{2}) = \left(-\frac{1}{2},-\frac{1}{6},\frac{7}{6}\right).
\end{align}
From this we find central charge and conformal dimensions $(c,\Delta_{1},\Delta_{2}) = \left(12,\tfrac{1}{3},\frac{5}{3}\right)$, and free parameters $(\mu_{1},\mu_{2}) = \left(-\tfrac{25}{36},-\tfrac{7}{72}\right)$. Thus far, we have only investigated the vacuum character and found the $q$-series expansion 
\begin{align}
    \chi_{0}(\tau) = q^{-\tfrac{1}{2}}\left(1 + 58q + 66q^{2} + \ldots\right).
\end{align}
In order to establish that this is indeed a valid character, we should check for positivity in higher-order Fourier coefficients and repeat the same process for the characters $\chi_{\tfrac{1}{3}}(\tau)$ and $\chi_{\tfrac{5}{3}}(\tau)$ in order to rule this as an admissible solution. The following is a general expression we obtain for the ratio $m_{1}$ from \ref{m_1_finding_equation},
\begin{align}
    m_{1}^{(i)} \equiv \frac{f_{1}^{(i)}}{f_{0}^{(i)}} = \ldots
\end{align}
where $i = 0,1,2$. From this we find $m_{1}^{(1)} = \ldots$








==> Two_character_Gamma_0_2+.tex <==
\section{Two-character theories for \texorpdfstring{$\Gamma_{0}^{+}(2)$}{Γ0(2)+}}\label{appendix:B}
The algorithm we follow to classify CFTs using MLDEs is the following:
\begin{enumerate}
    \item Postulate MLDE for values of $n$ and fix the number of free parameters $\mu_{i}$.
    \item Find the solutions to the MLDE as a power series in $q = e^{2\pi i\tau}$ of the form
    \begin{align}
        \chi_{i}(\tau) = q^{\alpha_{i}}\left(m_{0}^{(i)} + m_{1}^{(i)}q + m_{2}^{(i)}q^{2} + \ldots\right),
    \end{align}
    where the exponent $\alpha_{0} = -\tfrac{c}{24}$ is negative in a unitary theory.
    \item Set up recursion relations to obtain coefficients $m_{n}^{(i)}$ and vary the parameters of the equation to make sure these are non-negative integers.
    \item Verify that coefficients $m_{n}^{(i)}$ remain non-negative integers to higher orders in $q$. This test passes the character as an admissible one and the corresponding candidate theory to be viable.
    \item Check if the candidate CFT is actually a well-defined consistent theory.
\end{enumerate}
The general form of the MLDE for $n=2$ and $\ell\neq0$ reads
\begin{align}
    \left[\omega_{2\ell}(\tau)\mathcal{D}^{2} + \omega_{2\ell + 2}(\tau)\mathcal{D} + \omega_{2\ell + 4}(\tau)\right]f(\tau) = 0.
\end{align}
The free parameters $\mu_{i}$ in this MLDE come as coefficients to the modular forms and the number of them can be determined as follows
\begin{align}
        \#(\mu) =\text{dim}\mathcal{M}_{2\ell}(\Gamma_{0}^{+}(2)) + \text{dim}\mathcal{M}_{2\ell + 2}(\Gamma_{0}^{+}(2)) + \text{dim}\mathcal{M}_{2\ell + 4}(\Gamma_{0}^{+}(2)) -1.
\end{align}
We can rewrite the dimension formula for all $k\in2\mathbb{Z}$ and $k\not\equiv 2\ (\text{mod}\ 8)$ as $\text{dim}\ \mathcal{M}_{k}(\Gamma_{0}^{+}(2))\left\lfloor\left.\tfrac{k}{8}\right\rfloor\right. + 1 = \left\lfloor\left.\tfrac{k}{8} + \left\lfloor\left.\tfrac{k}{4}\right\rfloor\right. - \tfrac{k}{4}\right\rfloor\right. + 1$ (see \cite{Junichi}) so that we obtain the following expression for the number of free parameters
\begin{align}\label{number_of_parameters_Gamma_0_2+}
    \#(\mu) = \left\lfloor\left.\left\lfloor\left.\frac{\ell}{2}\right\rfloor\right. - \frac{\ell}{4}\right\rfloor\right. + \left\lfloor\left.\frac{1}{4} - \frac{\ell}{4} + \left\lfloor\left.\frac{\ell}{2}\right\rfloor\right.\right\rfloor\right. + 
    \left\lfloor\left.-\frac{1}{4} - \frac{\ell}{4} + \left\lfloor\left.\frac{\ell + 1}{2}\right\rfloor\right.\right\rfloor\right. + 2,\ 2\ell\not\equiv 2\ (\text{mod}\ 8).
\end{align}
We do this since this formula undercounts the same obtained via substituting \ref{basis_decomposition_Gamma_0_2+} for $k\not\equiv 2\ (\text{mod}\ 8), k\in2\mathbb{Z}$ by one unit. This is preferable since we do not consider the cusp form for any modular form $\omega_{2\ell + n}(\tau)$ in the analysis done below since inclusion of the same yields negative or fractional values for $m_{n}^{(i)}$ that would rule out the candidate theory. On the other hand, for the case of $k \equiv 2\ (\text{mod}\ 8), k\in2\mathbb{Z}$, we are to use the following expression
\begin{align}\label{number_of_parameters_Gamma_0_2+_2mod8}
    \#(\mu) = \left\lfloor\left.\frac{\ell}{4}\right\rfloor\right. + \left\lfloor\left.\frac{\ell + 1}{4}\right\rfloor\right. + \left\lfloor\left.\frac{\ell + 2}{4}\right\rfloor\right. -1,\  2\ell\equiv 2\ (\text{mod}\ 8).
\end{align}

\subsection*{\texorpdfstring{$\ell = 0$}{Lg}}
Let us consider the case with no poles $\ell = 0$ and two characters $n = 2$. The MLDE in this case reads
\begin{align}\label{MLDE_n=2_Fricke_2}
    \left[\mathcal{D}^{2} + \phi_{1}(\tau) \mathcal{D} + \phi_{0}(\tau)\right]f(\tau) = 0,
\end{align}
where $\phi_{0}(\tau)$ and $\phi_{1}(\tau)$ are modular forms of weights $4$ and $2$ respectively. The space $\mathcal{M}_{2}(\Gamma_{0}^{+}(2))$ is zero-dimensional and there are no modular forms of weight $2$ in $\Gamma_{0}^{+}(2)$. Hence, we set $\phi_{1}(\tau) = 0$. The space $\mathcal{M}_{4}(\Gamma_{0}^{+}(2))$ is one-dimensional and hence, we set $\phi_{0}(\tau) = \mu E_{4}^{(2^{+})}(\tau)$. For these choices, the second-order MLDE takes the following form
\begin{align}\label{MLDE_n=2_Gamma_0_2+}
    \left[\mathcal{D}^{2} + \mu E_{4}^{(2^{+})}(\tau)\right]f(\tau) = 0,
\end{align}
where $\mu$ is an independent parameter. Now, since the covariant derivative transforms a weight $r$ modular form into one of weight $r+2$, the double covariant derivative of a weight $0$ form is
\begin{align}
    \begin{split}
        \mathcal{D}^{2} = \mathcal{D}_{(2)}\mathcal{D}_{(0)} =& \left(\frac{1}{2\pi i}\frac{d}{d\tau} - \frac{1}{4}E^{(2^{+})}_{2}(\tau)\right)\frac{1}{2\pi i}\frac{d}{d\tau}\\
        =& \Tilde{\partial}^{2} - \frac{1}{4}E^{(2^{+})}_{2}(\tau)\Tilde{\partial}.
    \end{split}
\end{align}
The MLDE \ref{MLDE_n=2_Gamma_0_2+} now reads
\begin{align}\label{MLDE_n=2_Gamma_0_2+_expanded}
    \left[\Tilde{\partial}^{2} - \frac{1}{4}E^{(2^{+})}_{2}(\tau)\Tilde{\partial} + \mu E_{4}^{(2^{+})}(\tau)\right]f(\tau) = 0.
\end{align}
This equation can be solved by making the following mode expansion substitution for the character $f(\tau)$ and the other modular forms,
\begin{align}\label{series_defs_Gamma_0_2+}
    \begin{split}
        f(\tau) =& q^{\alpha}\sum\limits_{n= 0}^{\infty}f_{n}q^{n},\\
        E_{k}(\tau) =& \sum\limits_{n=0}^{\infty}E_{2,n}^{(2^{+})}q^{n}\\
        =& 1 - 8 q - 40 q^2 - 32 q^3 - 104 q^4 + \ldots,\\
        E_{4}^{(2^{+})}(\tau) =& \sum\limits_{n=0}^{\infty}E_{4,n}^{(2^{+})}q^{n}\\
        =& 1 + 48 q + 624 q^2 + 1344 q^3 + 5232 q^4 + \ldots
    \end{split}
\end{align}
Substituting these expansions in the MLDE, we obtain
\begin{align}\label{MLDE_mode_Gamma_0_2+}
    q^{\alpha}\sum\limits_{n=0}^{\infty}f_{n}q^{n}\left[(n+\alpha)^{2} - (n + \alpha)\sum\limits_{m=0}^{\infty}\frac{1}{4}E^{(2^{+})}_{2,m}q^{m} + \mu\sum\limits_{m=0}^{\infty} E_{4,m}^{(2^{+})}q^{m}\right] = 0.
\end{align}
When $n=0,m=0$, with $E^{(2^{+})}_{2,0} = E^{(2^{+})}_{4,0} = 1$, we obtain the following indicial equation
\begin{align}
    \alpha^{2} -\frac{1}{4} \alpha +  \mu = 0.
\end{align}
The parameter $\mu$ can now be fixed using this equation. Let us denote the roots of this equation, in increasing order, as $\alpha_{0}$ and $\alpha_{1}$. Solving this indicial equation gives us
\begin{align}\label{roots_n=2_l=0_Gamma_0_2+}
    \begin{split}
        \alpha_{0} =& \frac{1}{8}\left(1 - \sqrt{1 - 64\mu}\right) = \frac{1}{8}(1 - x),\\
        \alpha_{1} =& \frac{1}{12}\left(1 + \sqrt{1 - 64\mu}\right) \equiv \frac{1}{8}(1 + x),
    \end{split}
\end{align}
where we have set $x = \sqrt{1 - 64\mu}$. The smaller solution $\alpha_{0} = \tfrac{1}{8}(1-x)$ corresponds to the identity character which behaves as $f(\tau) \sim q^{\tfrac{1-x}{8}}\left(1 + \mathcal{O}(q)\right)$. We know that the identity character $\chi_{0}$, associated with a primary of weight $\Delta_{0} = 0$ behaves as $\chi_{0}\sim q^{-\tfrac{c}{24}}\left(1 + \mathcal{O}(q)\right)$. Comparing the two behaviours, we obtain the following expression for the central charge
\begin{align}\label{central_charge_x}
    c = 3(x-1).
\end{align}
To find the conformal dimension $\Delta$, we compare the behaviours with the larger solution for $\alpha$, i.e. $f(\tau)\sim q^{\tfrac{1 + x}{8}}\left(1  +\mathcal{O}(q)\right)$ and $\chi\sim q^{-\tfrac{c}{24} + \Delta}\left(1 + \mathcal{O}(q)\right)$. This gives us
\begin{align}
    \Delta = \frac{x}{4}.
\end{align}
Next, to obtain a recurrence relation among the coefficients $f_{n}$, we use the Cauchy product of two infinite series which reads
\begin{align}
    \left(\sum\limits_{i=0}^{\infty}\alpha_{i}\right)\cdot\left(\sum\limits_{j=0}^{\infty}\beta_{j}\right) = \sum\limits_{k=0}^{\infty}\gamma_{k},\ \gamma_{k} = \sum\limits_{p=0}^{k}\alpha_{p}\beta_{k-p}.
\end{align}
This gives us
\begin{align}
    \begin{split}
         \left(\sum\limits_{m=0}^{\infty}E^{(2^{+})}_{4,m}(\tau)q^{m}\right)\left(\sum\limits_{n=0}^{\infty}f_{n}q^{n}\right) =& \sum\limits_{k=0}^{\infty}\left(\sum\limits_{p=0}^{k}E^{(2^{+})}_{4,m}f_{k-p}\right)q^{k},\\
        \left(\sum\limits_{m=0}^{n}E^{(2^{+})}_{2,m}q^{m}\right)\left(\sum\limits_{n=0}^{\infty}f_{n}q^{n}(n+\alpha)\right) =& \sum\limits_{k=0}^{\infty}\left(\sum\limits_{p=0}^{k}E^{(2^{+})}_{2,p}(k+\alpha - p)f_{k-p}\right)q^{k}.
    \end{split}
\end{align}
Substituting this back into the MLDE, we get
\begin{align}\label{recursion_l=0_Gamma_0_2+}
    f_{n} = \left((n + \alpha)^{2} - \frac{1}{4}(n + \alpha) + \mu\right)^{-1}\sum\limits_{m=1}^{n}\left(\frac{(n + \alpha - m)}{4}E^{(2^{+})}_{2,m} - \mu E^{(2^{+})}_{4,m}\right)f_{n-m}.
\end{align}
When $n = 1$, we solve for the ratio $\tfrac{f_{1}}{f_{0}}$ in terms of $\alpha$ with coefficients $E^{(2^{+})}_{2,1} = -8$ and $E_{4,1}^{(2^{+})} = 48$ to obtain 
\begin{align}
    m^{(i)}_{1} = \frac{f^{(i)}_{1}}{f^{(i)}_{0}} = \frac{8\alpha_{i}(-7 + 24\alpha_{i})}{3 + 8\alpha_{i}},
\end{align}
for $ i = 0,1$ corresponding to ratios of $m^{(0)}_{1}$ and $m^{(1)}_{1}$ taken with respect to values $\alpha_{0}$ and $\alpha_{1}$ respectively. Restricting to $i=0$ and assuming that $\alpha_{i} = -\tfrac{c}{24}$, we find
\begin{align}
    m_{1}^{(0)} = \frac{c(7+c)}{9-c}.
\end{align}
Dropping the script associated with the index $i$, we see that for $m_{1}\geq 0$, we require $c<9$. Rewriting this, we have
\begin{align}
    c^{2} + c(m_{1} + 7) = 9m_{1}.
\end{align}
This tells us that $c$ is an integer. Hence, for two character theories with $\ell = 0$, we have $c\in\mathbb{Z}$ and the bound $c< 9$. Solving the quadratic equation, we notice that for $c$ to be rational, the following determinant has to be rational
\begin{align}
    \sqrt{49 + 50m_{1} + m_{1}^{2}}.
\end{align}
Now, since we require $m_{1}\in\mathbb{Z}$, we must demand that the square root is an integer and this gives us
\begin{align}\label{recast_prior}
    \left(m_{1} + 25\right)^{2} - 576 = k^{2},
\end{align}
where $k^{2}\in\mathbb{Z}$. We define $p$ such that we shift $k$ by an integer amount that absorbs the first two terms on the left-hand side
\begin{align}
    p = 25 + m_{1} - k,
\end{align}
and we recast \ref{recast_prior} as follows
\begin{align}
    m_{1} + 25 = \frac{576 + p^{2}}{2p} = \frac{288}{p} + \frac{p}{2}.
\end{align}
This tells us that $p$ must be even and that it must divide $288$. Restricting $k$ to be positive, we see that we have $k\geq m_{1}$ which implies that $p<25$. We conclude that all possible values of $m_{1}$ are found by those values of $p$ below $26$ that divide $288$ and are even. The list of these values is $p = \{2,4,6,8,12,16,18,24,32,36,48,72,96,144\}$. We note that at $p = 24$, we obtain $(m_{1}, c, \Delta) = (-1, -3,0)$ which we ignore since we only want unitary theories, and the values $p = \{32,\ldots, 144\}$ yield the same result as that of $p = \{2,\ldots,18\}$ and hence, we ignore these to avoid double-counting. Table \ref{tab:theory_Fricke_2+} contains CFT data among other things that correspond to particular theories.
\begin{table}[htb!]
    \centering
    \begin{tabular}{||c|c|c|c|c||}
    \hline
    $p$ & $\mu$ & $m_{1}$ & $c$ & $\Delta$\\ [0.5ex]
    \hline\hline
    2  & $-\tfrac{7}{36}$ & 120 & 8 & $\tfrac{11}{12}$\\[0.5ex]
    4 & $-\tfrac{91}{576}$ & 49 & 7 & $\tfrac{5}{6}$\\[0.5ex]
    6 & $-\tfrac{1}{8}$ & 26 & 6 & $\tfrac{3}{4}$\\[0.5ex]
    8 &$-\tfrac{55}{576}$ & 15 & 5 & $\tfrac{2}{3}$\\[0.5ex]
    12 & $-\tfrac{3}{64}$ & 5 & 3 & $\tfrac{1}{2}$\\[0.5ex]
    16 & $-\tfrac{7}{576}$ & 1 & 1 & $\tfrac{1}{3}$\\[0.5ex]
    18 & $0$ & 0 & 0 & $\tfrac{1}{4}$\\[1ex]
    \hline
    \end{tabular}
    \caption{$c$ and $\Delta$ data corresponding to the Fricke group $\Gamma_{0}^{+}(2)$ for the choice $\phi_{0} = \mu E^{(2^{+})}_{4}(\tau)$ with $\ell = 0$.}
    \label{tab:theory_Fricke_2+}
\end{table}
\noindent
The ratio $m_{1}$ being non-negative is not sufficient proof to convince ourselves that this data might indeed be related to a CFT. Hence, we compute $m_{2}$ using recursion relation \ref{recursion_l=0_Gamma_0_2+}. If this turns out to be negative or fractional, then we rule out the theory as a viable candidate. We $n = 2$, we get
\begin{align}
     m_{2}^{(i)} \equiv \frac{f_{2}^{(i)}}{f_{0}^{(i)}} = \frac{4\alpha_{i}(312\alpha_{i} -83)}{8\alpha_{i} + 7} + \frac{4m_{1}^{(i)}(-1 + \alpha_{i}(-7 + 24\alpha_{i}))}{8\alpha_{i} + 7}.
\end{align}
The values of $m_{2}$ fr $i = 0$ is tabulated in table
\ref{tab:theory_Fricke_2+_m2}.
\begin{table}[htb!]
    \centering
    \begin{tabular}{||c|c|c||}
    \hline
    $p$ & $c$ & $m_{2}$\\ [0.5ex]
    \hline\hline
    2  & 8 & $\tfrac{6508}{13}$\\[0.5ex]
    4 & 7 & 173\\[0.5ex]
    6 & 6 & 79\\[0.5ex]
    8 & 5 & 40\\[0.5ex]
    12 & 3 & 11\\[0.5ex]
    16 & 1 & 2\\[0.5ex]
    18 & 0 & 0\\[1ex]
    \hline
    \end{tabular}
    \caption{Values of $m_{2}$ for corresponding to the Fricke group $\Gamma_{0}^{+}(2)$ for the choice $\phi_{0} = \mu E^{(2^{+})}_{4}(\tau)$ with $\ell = 0$.}
    \label{tab:theory_Fricke_2+_m2}
\end{table}
\noindent
We discard the case $p = 2$ since the coefficient turns out to be fractional. Furthermore, we also discard the case $p = 18$ since further computation yields all coefficients $m_{i}$ to be null valued which makes this a trivial solution. We have now restricted to cases $p = \{4,6,8,12,16\}$. Next, we compute $m_{3}$ using recursion relation \ref{recursion_l=0_Gamma_0_2+} and this turns out to be
\begin{align}
     m_{3}^{(i)} \equiv \frac{f_{3}^{(i)}}{f_{0}^{(i)}} = \frac{32\alpha_{i}(168\alpha_{i} -43)}{24\alpha_{i} + 33} + \frac{8m_{1}^{(i)}(-5 + \alpha_{i}(-83 + 312\alpha_{i}))}{24\alpha_{i} + 33} + \frac{8m_{2}^{(i)}(-2 + \alpha_{i}(-7 + 24\alpha_{i}))}{24\alpha_{i} + 33}.
\end{align}
\noindent
The integral values of $m_{3}$ for $i = 0$ are shown in table \ref{tab:theory_Fricke_2+_m3}
\begin{table}[htb!]
    \centering
    \begin{tabular}{||c|c|c||}
    \hline
    $p$ & $c$ & $m_{2}$\\ [0.5ex]
    \hline\hline
    6 & 6 & 326\\[0.5ex]
    8 & 5 & 135\\[0.5ex]
    12 & 3 & 20\\ [0.5ex]
    16 & 1 & 1\\[0.5ex]
    \hline
    \end{tabular}
    \caption{Values of $m_{3}$ for corresponding to the Fricke group $\Gamma_{0}^{+}(2)$ for the choice $\phi_{0} = \mu E^{(2^{+})}_{4}(\tau)$ with $\ell = 0$.}
    \label{tab:theory_Fricke_2+_m3}
\end{table}
\noindent
In a similar fashion, computing coefficients for $i = 0,1$, we obtain the coefficients of the two characters, which to order $\mathcal{O}(q^{6})$ for data $(c,\Delta)$ are shown below,
\begin{align}
        \begin{split}
        \left(1, \tfrac{1}{3}\right):&\begin{cases}
        \chi_{0} = q^{-\tfrac{1}{24}}\left(1 + q + 2q^{2} + q^{3} + 3q^{4} + 3q^{5} + \ldots\right),\\
        \chi_{\tfrac{1}{3}} = q^{\tfrac{7}{24}}\ \left(1 + q^{2} + q^{3} + 2q^{4} + q^{5} + \ldots\right),\\
        \end{cases}\\
        \left(3, \tfrac{1}{2}\right):&\begin{cases}
        \chi_{0} = q^{-\tfrac{1}{8}}\left(1 + 5q + 11q^{2} + 20q^{3} + 41q^{4} + 76q^{5} + \ldots\right),\\
        \chi_{\tfrac{1}{2}} = q^{\tfrac{3}{8}}\ \left(1 + q^{2} + 5q^{3} + 6q^{4} + 16q^{5} + \ldots\right),\\
        \end{cases}\\
        \left(5, \tfrac{2}{3}\right):&\begin{cases}
        \chi_{0} = q^{-\tfrac{5}{24}}\left(1 + 15q + 40q^{2} + 135q^{3} + 290q^{4} + 726q^{5} + \ldots\right),\\
        \chi_{\tfrac{1}{2}} = q^{\tfrac{11}{24}}\ \left(5 + 11q^{2} + 55q^{3} + 100q^{4} + 290q^{5} + \ldots\right),\\
        \end{cases}
        \end{split}
\end{align}
For the case $(6,\tfrac{3}{4})$, we find that the only the vacuum behaves well with an expansion $\chi_{0} = q^{-\tfrac{1}{24}}\left(1 + 26q + 76q^{2} + 326q^{3} + 755q^{4} + 2106q^{5} + \ldots\right)$.

==> Two_character_Gamma_0_7+.tex <==
\section{Two-character theories for \texorpdfstring{$\Gamma_{0}^{+}(7)$}{Γ0(7)+}}\label{appendix:D}
For the general form of the MLDE for $n=2$, the free parameters $\mu_{i}$ come as coefficients to the modular forms and the number of them can be determined as follows
\begin{align}\label{number_of_parameters_F}
    \begin{split}
        \#(\mu) =&\text{dim}\mathcal{M}_{2\ell}(\Gamma^{+}_{0}(7)) + \text{dim}\mathcal{M}_{2\ell + 2}(\Gamma^{+}_{0}(7)) + \text{dim}\mathcal{M}_{2\ell + 4}(\Gamma^{+}_{0}(7)) -1\\
        =& 2\left(\left\lfloor\left.\frac{\ell}{2}\right\rfloor\right. + \left\lfloor\left.\frac{\ell+1}{2}\right\rfloor\right. + \left\lfloor\left.\frac{\ell+2}{2}\right\rfloor\right.\right) + \left\lfloor\left.\frac{2\ell}{3}\right\rfloor\right. + \left\lfloor\left.\frac{2\ell+2}{3}\right\rfloor\right. + \left\lfloor\left.\frac{2\ell+4}{3}\right\rfloor\right. -3\ell -1.
    \end{split}
\end{align}

\subsubsection*{\texorpdfstring{$\ell=0$}{Lg}}
Consider the simple case with no poles $\ell = 0$ and two characters. The MLDE in this case reads
\begin{align}
    \left[\mathcal{D}^{2} + \phi_{1}(\tau)\mathcal{D} +  \phi_{0}(\tau) \right]f(\tau) = 0,
\end{align}
where $\phi_{0}(\tau)$ and $\phi_{1}(\tau)$ are modular forms of weights $4$ and $2$ respectively. Since there exists no weight $2$ modular form that belongs to the space of modular forms corresponding to the Fricke group $\Gamma_{0}^{+}(7)$, the MLDE simplifies to 
\begin{align}\label{MLDE_n=2}
    \left[\mathcal{D}^{2} + \phi_{0}(\tau)\right]f(\tau) = 0.
\end{align}
We now have three unique choices for $\phi_{0}(\tau)$, namely
\begin{align}\label{choices_phi}
    \begin{split}
        \phi_{0}(\tau) =& \mu E^{(7^{+})}_{4}(\tau) = \mu\Theta_{4,7}(\tau)\\
        =& \mu\left(1 + \tfrac{24}{5}q + \tfrac{216}{5}q^{2} + \tfrac{672}{5}q^{3} + \tfrac{1752}{5}q^{4} + \ldots\right)\\
        \phi_{0}(\tau) =& \mu \Theta^{2}_{2,7}(\tau) = \mu\theta_{7}^{4}(\tau)\\
        =& \mu\left(1 + 8q + 40q^{2} + 128q^{3} + 328q^{4} + \ldots\right)\\
        \phi_{0}(\tau) =& \mu\Delta_{7^{+},4}(\tau) = \mu\theta_{7}(\tau)j_{7}^{-1}(\tau)\mathbf{k}(\tau)\\
        =& \mu\left(q - q^{2} - 2q^{3} - 7q^{4} + \ldots\right).
    \end{split}
\end{align}
Here $\mu$ is a free parameter which will be fixed later. The space $\mathcal{M}_{4}\left(\Gamma_{0}^{+}(7)\right)$ is one-dimensional and we notice that all three of the above choices can be generated by $\Theta_{2,7}^{2}(\tau)$ and $\Theta_{4,7}(\tau)$ as shown below
\begin{align}
    \begin{split}
        E_{4}^{7^{+}}(\tau) =& a\Theta_{2,7}^{2} + b\Theta_{4,7}(\tau),\ a = 0,b = 1\\
        \Delta_{7^{+},4}(\tau) =& a\Theta_{2,7}^{2}(\tau) + b\Theta_{4,7}(\tau),\ a = \frac{5}{16},\ b = -\frac{5}{16}.
    \end{split}
\end{align}
Lastly, we note that $E_{4}^{(7^{+})}(\tau)$ is a quasi-modular form unlike $\Theta_{2,7}^{2}(\tau)$ (which is a modular form) since it transforms as follows under a modular transformation $\gamma = \tfrac{a\tau + b}{c\tau + d}$,
\begin{align}
    \begin{split}
        E_{k}(p\gamma(\tau)) =& (c\tau + d)^{2}E_{k}(p\tau) + \frac{12c}{2\pi ip}(c\tau + d),\\
        E_{4}^{(7^{+})}(\gamma(\tau)) =& (c\tau + d)^{2}E_{4}^{(7^{+})}(\tau) + \frac{48c}{25}\frac{(c\tau + d)}{2\pi i}.
    \end{split}
\end{align}
Hence, we only consider the second choice for $\phi_{0}(\tau)$ for our calculation. From the basis \ref{Fricke_basis}, we find
\begin{align}
    \begin{split}
        \mathcal{M}_{4}(\Gamma_{0}^{+}(7)) =& \theta_{7}(\tau)\left(\mathbb{C}\theta_{7}^{3}\oplus\mathbf{k}\mathbf{t}\right)\\
        =& \mathbb{C}\Theta_{2,7}^{2}\oplus\mathbb{C}\theta_{7}\mathbf{k}\mathbf{t}.
    \end{split}
\end{align}
Hence, the most general choice for $\phi_{0}(\tau)$ would be
\begin{align}
    \phi_{0}(\tau) =  \mu_{1}\Theta_{2,7}^{2}(\tau) + \mu_{2}\left(\theta_{7}\mathbf{k}\mathbf{t}\right)(\tau).
\end{align}
We now have two free parameters which matches with the result of \ref{number_of_parameters_F} for $\ell = 0$. Now, since the covariant derivative transforms a weight $r$ modular form into one of weight $r+2$, the double covariant derivative of a weight $0$ form is
\begin{align}
    \begin{split}
        \mathcal{D}^{2} = \mathcal{D}_{(2)}\mathcal{D}_{(0)} =& \left(\frac{1}{2\pi i}\frac{d}{d\tau} - \frac{1}{6}E_{2}(\tau)\right)\frac{1}{2\pi i}\frac{d}{d\tau}\\
        =& \Tilde{\partial}^{2} - \frac{1}{6}E_{2}(\tau)\Tilde{\partial}.
    \end{split}
\end{align}
The MLDE \ref{MLDE_n=2} now reads
\begin{align}
    \left[\Tilde{\partial}^{2} - \frac{1}{6}E_{2}(\tau)\Tilde{\partial} + \phi_{0}(\tau)\right]f(\tau) =0.
\end{align}
This equation can be solved by making the following mode expansion substitution for the character $f(\tau)$ and the Eisenstein series $E_{k}(\tau)$, and modular forms $\Theta_{2,7}^{2}(\tau)$ and $\left(\theta_{7}\mathbf{k}\mathbf{t}\right)(\tau)$,
\begin{align}\label{series_defs}
    \begin{split}
    f(\tau) =& q^{\alpha}\sum\limits_{n= 0}^{\infty}f_{n}q^{n},\\
    E_{k}(\tau) =& \sum\limits_{n=0}^{\infty}E_{k,n}q^{n},\\ \Theta_{2,7}^{2}(\tau) =& \sum\limits_{n=0}^{\infty}\Theta_{n}q^{n}\\
    =& 1 + 8 q + 40 q^2 + 128 q^3 + 328 q^4 + \ldots,\\
    \left(\theta_{7}\mathbf{k}\mathbf{t}\right)(\tau) =& \sum\limits_{n=0}^{\infty}\mathfrak{a}_{n}q^{n}\\
    =& 0 + q - q^2 - 2 q^3 - 7 q^4 + \ldots\\
    \end{split}
\end{align}
Substituting these expansions in the MLDE, we get
\begin{align}\label{MLDE_series_expressions}
    q^{\alpha}\sum\limits_{n=0}^{\infty}f_{n}q^{n}\left[\left(n + \alpha\right)^{2} + \sum\limits_{m=0}^{\infty}\left(\mu_{1}\Theta_{m} + \mu_{2}\mathfrak{a}_{m} - \frac{(n+\alpha)}{6}E_{2,m}\right)q^{m}\right] = 0.
\end{align}
We first restrict ourselves to the case when $\mu_{1} = \mu \neq 0$ and $\mu_{2} = 0$.
When $n=0, m=0$, with $E_{2,0} = 1 = \Theta_{0}$, we get the indicial equation
\begin{align}\label{alpha_eqn}
    \begin{split}
        &\alpha^{2} - \frac{\alpha}{6} + \mu = 0,\\
        &\alpha_{0} = \frac{1}{12}\left(1 -\sqrt{1 + 144\mu}\right) \equiv \frac{1}{12}\left(1 - x\right),\\
        &\alpha_{1} = \frac{1}{12}\left(1+\sqrt{1 + 144\mu}\right)\equiv \frac{1}{12}(1+x)
    \end{split}
\end{align}
where we set $x = +\sqrt{1 + 144\mu}$. The smaller solution $\alpha_{0} = \tfrac{1}{12}(1-x)$ corresponds to the identity character which behaves as $f(\tau) \sim q^{\tfrac{1-x}{12}}\left(1 + \mathcal{O}(q)\right)$. From \ref{character_behaviour}, the identity character $\chi_{0}$, associated with a primary of weight $\Delta_{0} = 0$ behaves as $\chi_{0}\sim q^{-\tfrac{c}{24}}\left(1 + \mathcal{O}(q)\right)$. Comparing the two behaviours, we obtain the following expression for the central charge
\begin{align}
    c = 2(x-1).
\end{align}
To find the conformal dimension $\Delta$, we compare the behaviours with the larger solution for $\alpha$, i.e. $f(\tau)\sim q^{\tfrac{1 + x}{12}}\left(1  +\mathcal{O}(q)\right)$ and $\chi\sim q^{-\tfrac{c}{24} + \Delta}\left(1 + \mathcal{O}(q)\right)$. This gives us
\begin{align}
    \Delta = \frac{x}{6}.
\end{align}
Next, to obtain a recurrence relation among the coefficients $f_{n}$, we use Cauchy product of two infinite series which reads
\begin{align}
    \left(\sum\limits_{i=0}^{\infty}\alpha_{i}\right)\cdot\left(\sum\limits_{j=0}^{\infty}\beta_{j}\right) = \sum\limits_{k=0}^{\infty}\gamma_{k},\ \gamma_{k} = \sum\limits_{p=0}^{k}\alpha_{p}\beta_{k-p}.
\end{align}
This gives us
\begin{align}\label{product_formulae}
    \begin{split}
        \left(\sum\limits_{m=0}^{\infty}E_{2,m}q^{m}\right)\left(\sum\limits_{n=0}^{\infty}f_{n}q^{n}(n+\alpha)\right) =& \sum\limits_{k=0}^{\infty}\left(\sum\limits_{p=0}^{k}E_{2,p}(k+\alpha - p)f_{k-p}\right)q^{k}\\
        \left(\sum\limits_{m=0}^{\infty}\Theta_{m}(\tau)q^{m}\right)\left(\sum\limits_{n=0}^{\infty}f_{n}q^{n}\right) =& \sum\limits_{k=0}^{\infty}\left(\sum\limits_{p=0}^{k}\Theta_{p}f_{k-p}\right)q^{k}.
    \end{split}
\end{align}
Relabelling and substituting this back into the MLDE, we get
\begin{align}
    \begin{split}
        q^{\alpha}\sum\limits_{n=0}^{\infty}q^{n}\left((n+\alpha)^{2} - \frac{(n+\alpha)}{6}E_{2,0} + \mu \Theta_{0}\right)f_{n} = q^{\alpha}\sum\limits_{n=0}^{\infty}q^{n}&\left(\sum\limits_{m=1}^{n}\left(\frac{1}{6}E_{2,m}(n+\alpha - m) - \mu\Theta_{m}\right)f_{n-m}\right).
    \end{split}
\end{align}
With $E_{k,0} = 1 = \Theta_{0}$ and \ref{alpha_eqn}, we get
\begin{align}\label{recursion_l=0}
    f_{n} = \left(n^{2} + 2\alpha n - \frac{n}{6}\right)^{-1}\sum\limits_{m=1}^{n}\left(\frac{1}{6}E_{2,m}(n+\alpha - m) - \mu\Theta_{m}\right)f_{n-m}.
\end{align}
When $n=1$ and $\alpha = \alpha_{0} = \tfrac{1}{12}(1-x)$, this simplifies to the following expression
\begin{align}
    \begin{split}
        m_{1}^{(0)}\equiv \frac{f_{1}^{(0)}}{f_{0}^{(0)}} = \frac{x^{2}+6x+7}{3(6-x)},
    \end{split}
\end{align}
where we used $E_{2,1} = -24$ and $\Theta_{1}= 8$. Solving for $x$, we obtain 
\begin{align}
    x = \frac{1}{2}\left(-(3m_{1} + 6) \pm \sqrt{(3m_{1}+6)^{2} + 4(18m_{1} + 7)}\right).
\end{align}
Since $2(x-1)$ is the central charge of the theory, $x$ must be rational. With $m_{1}^{(0)} = m_{1}$ and using the fact that $m_{1}$ is an integer, we conclude that at least one of the roots is rational. We now write
\begin{align}\label{to_be_recast}
    (3m_{1} + 18)^{2} - 260 = k^{2},
\end{align}
where $k\in\mathbb{Z}$. Defining
\begin{align}
    p \equiv 18 + 3m_{1} - k, 
\end{align}
we can recast \ref{to_be_recast} as follows
\begin{align}
   3m_{1} + 18 = \frac{p^{2} +260}{2p} = \frac{130}{p} + \frac{p}{2}.
\end{align}
This tells us that $p$ must be even, and that it must divide $130$. Restricting $k$ to be positive, we see that we have $k\geq 3m_{1}$ which implies that $p<18$. We conclude that all possible values of $m_{1}$ are found by those values of $p$ below $18$ that divide $130$ and that are even. The list of these values is $p = 2,10$. Table \ref{tab:theory_Fricke} contains CFT data among other things that correspond to particular theories.
\begin{table}[htb!]
    \centering
    \begin{tabular}{c|c|c|c|c}
    $p$ & $\mu$ & $m_{1}$ & $c$ & $\Delta$\\
    \hline & & & & \\
    2  & $\tfrac{1}{6}$ & 16 & 8 & $\tfrac{5}{6}$\\
    10 & $0$ & 0 & 0 & $\tfrac{1}{6}$\\
    \end{tabular}
    \caption{$c$ and $\Delta$ data corresponding to the Fricke group $\Gamma_{0}^{+}(7)$ for the choice $\phi_{0} = \mu\Theta_{2,7}^{2}(\tau)$ with $\ell = 0$.}
    \label{tab:theory_Fricke}
\end{table}
$m_{1}$ being non-negative is not sufficient proof to convince ourselves that this data might indeed be related to a CFT. Hence, we compute $m_{2}$ using recursion relation \ref{recursion_l=0}. If this turns out to be negative or fractional, then we rule out the theory as a viable candidate. We $n = 2$, we get
\begin{align}
    m_{2}^{(i)} \equiv \frac{f_{2}^{(i)}}{f_{0}^{(i)}} = -\frac{12(9\alpha_{i} + 10\mu)}{12\alpha_{i} + 11} - \frac{12m_{1}^{(i)}(3\alpha_{i} + 3 + 2\mu)}{12\alpha_{i} + 11}.
\end{align}
For $i = 0$, we find the values of $m_{2}^{(0)}$ corresponding to our candidate theories to yield $0$ for $p = 10$ and a negative fraction for $p = 2$ which we rule out. Now, we proceed to check if $m_{3}^{(i)}$ is positive as well for the surviving candidate theory. For $n = 3$, the recursion relation \ref{recursion_l=0} yields
\begin{align}
     m_{3}^{(i)} \equiv \frac{f_{3}^{(i)}}{f_{0}^{(i)}} = -\frac{32(3\alpha_{i} + 8\mu)}{12\alpha_{i} + 17} - \frac{8m_{1}^{(i)}(9\alpha_{i} + 9 + 10\mu)}{12\alpha_{i} + 17} - \frac{8m_{2}^{(i)}(3\alpha_{i} + 6 + 2\mu)}{12\alpha_{i} + 17}.
\end{align}
For $i = 0$, we obtain $m_{3}^{(0)} = \tfrac{224}{39}$ which is fractional and thus, we rule out this theory. We have found that there exists no CFT at $n = 2$ and $\ell = 0$.\\\\

\noindent For the case of $\mu_{1}\neq 0$ and $\mu_{2} \neq 0$, from \ref{MLDE_series_expressions} we find the following expressions for the free parameters by matching order by order in $q$
\begin{align}
    \begin{split}
        \mathcal{O}(1):&\ \mu = \frac{n + \alpha_{i}}{6} - (n + \alpha_{i}),\\
        \mathcal{O}(q):&\ \mu_{2} = \frac{8}{3}\left(3\alpha_{i}^{2} - 2\alpha_{i}\right).
    \end{split}
\end{align}
for $i=0,1$. When $i=0$, $\alpha_{0} = -\tfrac{c}{24}$ and this fixes
\begin{align}
    \mu_{1} = -\frac{c(c+4)}{576},\ \mu_{2} = \frac{c^{2}+16c}{72}.
\end{align}
From \ref{central_charge_valence_Fricke}, for $n = 2,\ \ell = 0$, we have $-\tfrac{c}{12} + \Delta = \tfrac{2}{3}$ which fixes the conformal dimension to be $\Delta = \tfrac{8 + c}{12}$. But it turns out that this case too yields inadmissible solutions. This makes sense since the parameter $\mu_{2}$ is one that is associated with a cusp form which, as we have seen in multiple instances in this work, is notorious for rendering the solutions to be inadmissible.


==> Two_character_MLDE_Fricke.tex <==
\section{Two-character MLDEs for Fricke groups}\label{sec:Two-character_Fricke}
As for the case of higher-character theories, we ought to be careful in the formulation of the MLDE for higher-character theories since the form of the Ramanujan-Serre covariant derivative would change. We will now expand on this. Consider an $(n+1)$-dimensional square matrix made up of $\chi_{0},\chi_{1},\ldots,\chi_{n-1},f$ and their derivatives. The most general ODE that is invariant under $\Gamma_{0}^{+}(p)$ reads
\begin{align*}
    \left[\omega_{2\ell}(\tau)\mathcal{D}^{n} + \omega_{2\ell + 2}(\tau)\mathcal{D}^{n-1} + \ldots + \omega_{2(n-1+\ell)}(\tau)\mathcal{D} + \omega_{2(n+\ell)}(\tau)\right]f(\tau) = 0,
\end{align*}
where the functions $\omega_{k}$ are holomorphic modular forms of weight $k$ and the derivatives here are the Ramanujan-Serre covariant derivatives given by
\begin{align}\label{Ramanujan-Serre}
    \begin{split}
        \mathcal{D} \equiv& \frac{1}{2\pi i}\frac{d}{d\tau} - \kappa(r) E^{(p^{+})}_{2}(\tau),\\
        \mathcal{D}^{n} =& \mathcal{D}_{r+2n-2}\circ\ldots\circ\mathcal{D}_{r+2}\circ\mathcal{D}_{r},
    \end{split}
\end{align}
where $r$ is the weight of the modular form on which the derivative acts and $\kappa(r)$, which is obtained from the valence formula, is tabulated in \ref{tab:Fricke_valence}.
\\
\begin{table}[htb!]
    \centering
    \begin{tabular}{||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c||}
    \hline
    $p$ & 2 & 3 & 5 & 7 & 11 & 13 & 17 & 19 & 23 & 29 & 31 & 41 & 59 & 71\\ [0.5ex]
    \hline\hline
    $\kappa(r)$ & $\tfrac{r}{8}$ & $\tfrac{r}{6}$ & $\tfrac{r}{4}$ & $\tfrac{r}{3}$ & $\tfrac{r}{2}$ & $\tfrac{7r}{12}$ & $\tfrac{3r}{4}$ & $\tfrac{5r}{6}$ & $r$ & $\tfrac{5r}{4}$ & $\tfrac{4r}{3}$ & $\tfrac{7r}{4}$ & $\tfrac{5r}{2}$ & $3r$\\ [1ex]
    \hline
    \end{tabular}
    \caption{Values computed using data in tables \ref{tab:Fricke_indices}, \ref{tab:correct_data}. Also see \cite{Junichi_extended} for explicit valence formulae for levels $p = 13,17,19$.}
    \label{tab:Fricke_valence}
\end{table}
\\
Note that the Fricke groups considered here do not possess any modular form of weight $2$, this can be seen from the dimension of the space of modular forms. The covariant derivative constructed here transforms a weight $r$ modular form to a weight $r+2$ modular form. Since each Fricke group has a distinct valence formula, each Fricke level would have a different formulation of the Ramanujan-Serre covariant derivatives. Let us now show the difference between the $\text{SL}(2,\mathbb{Z})$ Serre-Ramanujan covariant derivatives and those in Fricke groups. The $\text{SL}(2,\mathbb{Z})$ covariant derivative is defined as follows
\begin{align}\label{Ramanujan-Serre_SL2Z}
    \mathcal{D}_{\Gamma(1)} \equiv& \frac{1}{2\pi i}\frac{d}{d\tau} - \frac{r}{12}E_{2}(\tau).
\end{align}
Consider now the Eisenstein series of a Fricke group of level $p\in\mathbb{P}$ and weight $k$ is given by 
\begin{align}
    E^{(p^{+})}_{k}(\tau)\equiv \frac{p^{\tfrac{k}{2}}E_{k}(p\tau) + E_{k}(\tau)}{p^{\tfrac{k}{2}} + 1}.
\end{align}
Using this in \ref{Ramanujan-Serre} with $k = 2$, we find
\begin{align}
    \mathcal{D}_{\Gamma^{+}_{0}(p)} \equiv& \left(\frac{1}{2\pi i}\frac{d}{d\tau} - \frac{\kappa(r)}{p + 1}E_{2}(\tau)\right) - \frac{\kappa(r)}{p + 1}E_{2}(p\tau).
\end{align}
Since $p\neq 1$ and no $\kappa(r)$ value corresponding to a prime level $p$ conspires with $\tfrac{1}{p+1}$ to yield the desired factor of $\tfrac{r}{12}$, it is simply impossible to express the derivatives $\mathcal{D}_{\Gamma^{+}(p)}$ in terms of $\mathcal{D}_{\Gamma(1)}$. It turns out that we obtain the factor $\tfrac{r}{12}$ in \ref{Ramanujan-Serre_SL2Z} only at the Fricke level $N = 12$. The Eisenstein series of weight $2$ at this level is defined as follows \cite{Junichi}
\begin{align}
    E_{2,12^{+}}(\tau)\equiv \frac{12E_{2}(12\tau) - 6E_{2}(6\tau) + 4E_{2}(4\tau) + 3E_{2}(3\tau) - 2E_{2}(2\tau) + E_{2}(\tau)}{4}.
\end{align}
Using this in \ref{Ramanujan-Serre}, with $\kappa(r) = \tfrac{r}{2}$, we find
\begin{align}\label{Gamma_12+_derivative}
    \begin{split}
        \mathcal{D}_{\Gamma^{+}_{0}(12)} \equiv& \left(\frac{1}{2\pi i}\frac{d}{d\tau} - \frac{r}{12}E_{2}(\tau)\right) - \frac{r}{12}\left(12E_{2}(12\tau) - 6E_{2}(6\tau) + 4E_{2}(4\tau) + 3E_{2}(3\tau) - 2E_{2}(2\tau)\right)\\
        =& \mathcal{D}_{\Gamma(1)} - \frac{r}{12}\mathcal{E}_{2}(\tau),
    \end{split}
\end{align}
where $\mathcal{E}_{2}(\tau)$ contains the other weight $2$ Eisenstein series. From this brief discussion, we see that when we deal with the MLDEs of higher-character theories, it is important to consider the Eisenstein series associated with the Fricke group in building the covariant derivatives although they are built out
$\text{SL}(2,\mathbb{Z})$ Eisenstein series. It is easy to see from \ref{Gamma_12+_derivative} that the other terms in $\mathcal{E}_{2}(\tau)$ can have considerable influence on the solutions to the MLDE. Solving the $(n,\ell) = (2,0)$ MLDE for $\Gamma_{0}^{+}(2)$ with $\mathcal{D}_{\Gamma(1)}$ instead of $\mathcal{D}_{\Gamma_{0}^{+}(2)}$ yields spurious solutions. The $(n,\ell) = (2,0)$ MLDE analysis for the case of $\Gamma_{0}^{+}(2)$ is shown in appendix \ref{appendix:B}.
